Exposures Exposed: A Measurement and User Study to Assess Mobile Data Privacy in Context

Mobile devices have access to personal, potentially sensitive data, and there is a large number of mobile applications and third-party libraries that transmit this information over the network to remote servers (including app developer servers and third party servers). In this paper, we are interested in better understanding of not just the extent of personally identifiable information (PII) exposure, but also its context i.e., functionality of the app, destination server, encryption used, etc.) and the risk perceived by mobile users today. To that end we take two steps. First, we perform a measurement study: we collect a new dataset via manual and automatic testing and capture the exposure of 16 PII types from 400 most popular Android apps. We analyze these exposures and provide insights into the extent and patterns of mobile apps sharing PII, which can be later used for prediction and prevention. Second, we perform a user study with 220 participants on Amazon Mechanical Turk: we summarize the results of the measurement study in categories, present them in a realistic context, and assess users' understanding, concern, and willingness to take action. To the best of our knowledge, our user study is the first to collect and analyze user input in such fine granularity and on actual (not just potential or permitted) privacy exposures on mobile devices. Although many users did not initially understand the full implications of their PII being exposed, after being better informed through the study, they became appreciative and interested in better privacy practices.

==> exposures_exposed_soups21 arxiv-2/01-intro.tex <==
\section{Introduction}
%\red{TODO: change AntShield variable in main.tex for double-blind + something that makes more sense for this paper}

Mobile devices  have access to a wealth of personal, potentially sensitive information and there is a growing number of applications that access, process and transmit some of this information over the network. Sometimes this is necessary for the intended operation of the applications (\eg location is needed by {\em Google Maps}) and controllable (\eg by the user  through permissions),  but for the most part, users are not in control of their data today. Applications and third party libraries  routinely transmit user data to remote servers, including application servers but also ad servers and trackers, and users have typically limited visibility and understanding of what part of their personal data is shared, with whom, and for what purpose.

With the increased interest in online privacy, there are several bodies of related work. On one hand, a number of systems have been proposed that improve data transparency and protect  personally identifiable information (PII). In general, these systems fall into three categories: (i) static analysis and application re-writing \cite{nanfinding2018, gibler2012androidleaks, egele2011pios}, (ii) dynamic analysis with a modified or rooted OS \cite{enck2014taintdroid, phonelab, vallina2013rilanalyzer, falaki2010first, wei2012profiledroid}, and (iii) VPN-based network monitoring \cite{meddle, antmonitor-poster-mobicom15, razaghpanah2015haystack, song2015privacyguard, recon15, antmonitor-arxiv, antshield-arxiv}. While these tools provide more fine-grained control over sensitive data (as opposed to just permissions), the way users engage with these privacy-preserving systems is less well studied. 
On the other hand, in the human\text{-}computer interaction (HCI) community, researchers have extensively studied how different designs for app permissions affect users' decisions on which apps to install and which permission requests are considered legitimate by users \cite{Ismail2017, Jorgensen2015, wang2015investigating, almuhimedi2015your, Lin2012}. 
%\footnote{\magenta{Hence, there is a discrepancy between the tools being built in the systems community and the user studies being conducted in the HCI community. Specifically, although the systems community has built tools that transcend coarse-grained permissions, the user studies remain focused on the permissions model.} \magenta{[is that true? Check other user studies, e.g. last narseo's NDSS and recent Ubicomp and PETS user studies]}. Do we have new findings or just most recent or...?}
 A detailed review of related work is provided in Section \ref{sec:related}.

%In this paper, we attempt to close this gap by evaluating \anteater \cite{antmonitor15, antmonitor-poster-mobicom15, antmonitor-arxiv} -- one of the VPN-based tools that provides users with transparency and control over their PII. 

In this paper, we are interested in understanding {\em privacy exposures}, which we define as PII transmitted by a mobile app (or third party library used by the app) on the device, over the network interface, towards a remote server. Our goal is to understand not only the extent and mechanisms of PII exposure, but also its context (\ie functionality of the app, destination server, encryption used, frequency, etc.) and the risk perceived by mobile users today. For example, location needs to be shared for  a navigation app to perform its intended and legitimate function, and should not be of concern to the user. In contrast, if the same navigation app uses a library that shares device ids with a third-party server, this is more likely a privacy {\em leak}\footnote{Most prior work \cite{recon15, vallina2018tracking, antmonitor-poster-mobicom15} refers to PII found in outgoing packets as a ``privacy leak,'' because PII is by definition private information and an outgoing packets indicates exfiltration or a ``leak.'' However, we purposely distinguish between ``privacy exposure'' (a PII contained in an outgoing packet) and ``privacy leak'' (which is an exposure that is not necessary for the intended  functionality of the app, and/or goes to a third party server, or happens in clear text). This distinction, between a PII exposure and an actual leak, can only be made based on the {\em context}, which is one of the main aspects we investigate in this paper.}
   and should be of concern to the user. We are also interested in PII actually exposed in real network traffic, as opposed to potential privacy exposures as captured by permissions. To that end, we make the following two contributions.









%We  analyze the datasets that we collected from scratch, a) manually by testing the top 100 apps, and b) automatically by running automated scripts for top 400 apps and present the findings. Next, we demonstrate the results of a survey we conducted online where we asked real users how concerned they are with sharing their mobile data and how they understand privacy. Additionally, we crowdsourced labels for leaks based on our dataset in order to distinguish what type of information is needed for an app's functionality and what is potentially harmful when it is shared with remote servers.

%Prior work on crowdsourcing user's privacy awareness on mobile apps includes mostly studying privacy settings and preferences (\cite{Lin2012}, \cite{Jorgensen2015}, \cite{Ismail2017}). Our exploratory user study focuses on participants' reactions for certain information types that are destined to remote servers (analytics/ads and app developer).
 
% Prior work on improving data transparency and identifying potential privacy leaks includes static and dynamic analysis and network-centric approaches. %
%  In this paper, we take the latter approach: personal information  leaks happen, by definition, over network traffic, therefore a natural and comprehensive vantage point to identify and control leaks is at the network layer. Traffic can be monitored in the middle of the network (as in \meddle  \cite{meddle} and \recon \cite{recon15})  and/or on the device  itself (as in  \anteater \cite{antmonitor-arxiv}\cite{antmonitor-poster-mobicom15} and \textvtt{Lumen}  (a.k.a.  \haystack) \cite{razaghpanah2016haystack}).  A key challenge for network-based monitoring is how to analyze traffic both efficiently and securely.  The current state-of-the-art consists of the following complementary approaches. On one hand, \anteater \cite{antmonitor-arxiv} and  \textvtt{Lumen}  \cite{razaghpanah2016haystack} detect leaks on the device, but require a blacklist of strings (potential PII leaks) known a priori to search for. Therefore, they are unable to detect leakage of information that changes dynamically or is not part of the list.  On the other hand, \recon \cite{recon15} recently addressed this limitation, by training classifiers in a fully centralized way. However, the implementation relied on a trusted, remote proxy to route and analyze traffic, which potentially impacts scalability and security. %
 
%We adopt the on-device network monitoring paradigm, which presents both opportunities and challenges. On the upside, it  obviates the need for a trusted infrastructure and gives full control to the user, which we believe is the right approach in privacy. Devices also have access to important contextual information, such as certain personal information available on the phone, and which apps are responsible for transmitting packets.
%
%On the downside, mobile devices have limited resources to conduct traffic analysis, including deep packet inspection (DPI),  and training and applying machine learning classifiers for inferring leaks of PII. It is currently an open question as to how to train machine learning classifiers to retain high accuracy in a truly distributed manner. 
  
%In this paper, we take the first step towards enabling  distributed learning of personal information leaks from network traffic.  We present \antshield\xspace - a system that performs efficient on-device analysis,  provides accurate and comprehensive data privacy protection, and gives users  transparency and control over their personal information in real-time. 
  %
 % A key insight  is the distinction between PII that is \preDefLeak by the user or is readily available on the device, from PII  that is a priori \unknownLeak and should be  inferred by classifiers.  We  propose a hybrid  \stringMatch-classification approach:  %
 % (i) we build on  the \antLib \cite{antmonitor-arxiv} for intercepting packets on the device and looking for \preDefLeak strings in real-time and (ii) we build classifiers for the remaining \unknownLeak PII. 


{\em Measurement Study.} First, we utilize a state-of-the-art mobile network monitoring tool, \anteater \cite{antmonitor-arxiv}, to intercept and inspect outgoing packets transmitted over the mobile device's network interface.  Using \anteater, we conduct two extensive and systematic experiments (one manual and one automated) on Android phones, where we test 400 most popular Android apps (as of March 2017) and we collect 47,076 outgoing packets. We identify whether these packets contain any of 16 predefined types of PII (defined in Section \ref{sec:system}), together with related information, which we collectively refer to as {\em context} including: the destination server/domain  (\ie whether it is an App Developer server or a third-party Advertisers \& Analytics server), the app category (games, shopping, navigation \etc) which reveals the intended functionality of the app, whether the PII is exposed in clear text or is encrypted, and whether the app runs in the background or foreground.   Our datasets partly confirm findings of previous measurement studies 
%larger and 
of mobile devices but are richer: \eg they contain previously unseen exposures over plain TCP and UDP, exposures while the app is in the background, and malicious scanning for rooted devices.  We analyze our datasets and provide insights into the extent and nature of how PII is exposed today.  We also identify 
behavioral patterns, such as communities of domains and mobile apps involved in exposing private information. These patterns can be used in the future to design automated  prediction and prevention methods. We plan to make the datasets available to the community.




{\em User Study.} Second, we perform a user study on Amazon Mechanical Turk (MTurk) with \numUsers users. We  summarize the results of the measurement study in categories, present participants with real-world scenarios of private information exposure in context (type of PII, whether it is shared with the application or a third party, use of encryption, \etc) and we ask them  to assess the legitimacy (\ie whether the information is needed for the app's functionality) and privacy risk posed. We also educate the participants on how a single piece of PII can lead to even more information being discovered when combined with data fetched from a data broker. Finally, we ask users before and after the survey what actions they would be willing to take to protect their privacy, including using free/paid privacy-enhancing tools and contributing their data to crowdsourcing. 
%Our user study on MTurk provides insight into how many of the collected privacy exposures are actually leaks, \ie illegitimate exposures that are not needed for the app's functionality. 
%\footnote{\blue{Our main findings show that users are not familiar with how PII is shared across different apps, but they are willing to learn more. In particular, they are more concerned about protecting their phone number than other unique identifiers. Overall, users seem to appreciate our short tutorial about mobile privacy and they seek for a solution that would protect their data.} }
To the best of our knowledge, our user study is the first to collect and analyze user input in such {\em fine granularity} (\ie taking context into account) and on {\em actual} (not just potential or permitted) privacy exposures from mobile devices. We found that (i) many users did not initially understand the full implications of their PII being exposed but (ii) after being better informed through the study, they became appreciative and interested in better privacy practices. The insights gained by the study can inform the design of fine-grained data transparency and privacy preserving tools such as \anteater \cite{antmonitor-page}. 

%First, we perform a measurement study: we collect a new dataset via manual and automatic testing and capture the exposure of 16 PII types from 400 most popular Android apps. We analyze these exposures and provide insights into the extent and patterns of mobile apps sharing PII, which can be later used for prediction and prevention. Second, we perform a user study with 220 participants on Amazon Mechanical Turk: we summarize the results of the measurement study in categories, present them in a realistic context, and assess users? understanding, concern, and willingness to take action. To the best of our knowledge, our user study is the first to collect and analyze user input in such fine granularity and on actual (not just potential or permitted) privacy exposures on mobile devices. Although many users did not initially understand the full implications of their PII being exposed, after being better informed through the study, they became appreciative and interested in better privacy practices.

%%%%%%%%%%%%%%%%





The structure of the rest of the  paper is as follows. Section \ref{sec:related} reviews related work.
%
%Section \ref{sec:system} describes our system's rationale, design and implementation. %
 Section \ref{sec:data} describes the measurement study,  including the data collection, summary and analysis. Section \ref{sec:user_study} presents the Amazon Mechanical Turk study, based on our datasets. Section \ref{sec:conclusion} concludes  the paper and outlines directions for future solutions based on the findings of this study. 

==> exposures_exposed_soups21 arxiv-2/03-data.tex <==
\section{Measurement Study: Data Collection \& Analysis} \label{sec:data}

\input{03-system}

\input{04-1-datasets}

\input{04-3-datafindings} 



==> exposures_exposed_soups21 arxiv-2/03-system.tex <==
\subsection{Data Collection System: \antShield} \label{sec:system}



We are interested in collecting real-world cases of PII exposure, as captured in packet traces of outgoing packets (as opposed to potential exposures \eg indicated by permissions). We focus on PII that have been previously defined in related work (\eg \cite{recon15, razaghpanah2015haystack}). Specifically, we are interested in detecting PII that belong to the following list:

%{\bf Problem Statement.} Mobile devices have access to a wealth of resources and information, much of which is personal and potentially sensitive. We will refer to such  personally identifiable information as {\em PII}. Examples include:
%
\begin{itemize}
%
\item Device Identifiers: IMEI, IMSI, Android ID, phone number, serial number, ICCID, MAC Address, available through Android APIs.
%
\item User identifiers: usernames and passwords used to login to various apps (unavailable through Android APIs); Advertiser ID, email (available through Android).
%
\item User demographic:  first and last name, gender, zipcode, city, \etc \xspace - unavailable through Android APIs.
\item Location:  latitude and longitude coordinates, available through Android APIs.
%
%\item User-defined: the user can also define any custom string that should be monitored  (\eg see GUI in Fig. \ref{fig:guiPI}), such as digits of her credit card.
%
%
\end{itemize} 

 \begin{figure}[t!]
	\begin{center}
		\subfigure[\antShield Architecture. Data collection consists of the following steps: each packet is intercepted by \antLib, searched for any PII, and mapped to an app]{\includegraphics[width=0.99\linewidth]{figs/AntShieldSystem.pdf}\label{fig:antShield}\hspace{10pt}}
		\subfigure[PII, including those manually entered (name)]{\hspace{6pt}\includegraphics[width=0.7\linewidth]{figs/screenPI.png}\label{fig:guiPI}}
		%\vspace{-10pt}
		\caption{\antShield System used for Data Collection: Architecture and Screenshot.} %(building on top of \antLib v0.1.5).}%(a)(b) apply to all uses of the app. (c-f) are specific to Privacy Leaks.  (f) shows which apps send packets  to which IP destinations for all active connections and is updated in real-time.}%  \blind{A video and more details can be found on our website}%
		\label{fig:system}
		%\vspace{-15pt}
	\end{center}   
\end{figure}

To collect real cases of when the PII defined above are exposed, we build on \anteater, an app that intercepts all network traffic from the device without requiring rooting. We pick \anteater since it is a representative VPN-based tool for privacy protection (see Sec. \ref{sec:related}) and it is easy to extend it for data collection. The traffic interception, along with several utility functions of \anteater have been made available as a library, and we will refer to it as the \antLib \cite{antmonitor-arxiv, antmonitor-page}. We will refer to our data collection app that extends the \antLib, as \antShield \cite{antshield-arxiv, antmonitor-page, spawc_shuba}.\footnote{The design and performance evaluation of the \antShield system is a contribution on its own. However, we consider it out of the scope of this paper. Here, we only use \antShield as a tool to collect the packet traces that are the starting point of our measurement and user studies. } As shown in Fittg. \ref{fig:antShield}, \antShield receives outgoing packets via the \textvtt{PacketFilter} interface provided by the \antLib. Note that the \antLib also implements a TLS proxy, which allows it to decrypt SSL/TLS traffic of applications that do not use certificate pinning (see \cite{antmonitor-arxiv} for details). These decrypted packets are also passed to \antShield via the \textvtt{PacketFilter} interface. Each intercepted packet (unencrypted or decrypted) is searched for PII using the \antLib's Deep Packet Inspection (DPI) module. This module implements the Aho-Corasick search algorithm to find multiple strings in one pass of a given packet. Some of the PII defined above are available to all apps via Android APIs and are thus easy to find in packets. To find PII that are unavailable through APIs, we add them to the list of strings to search for using \antshield's GUI -- see Fig. \ref{fig:guiPI}. Note that this methodology may miss PII that are obfuscated by applications prior to transmission, but as shown in \cite{continella2017obfuscation} such behavior is rare. After DPI, we use the \antLib's \textvtt{mapPacket} API call to note which app was responsible for generating the outgoing packet in question. Finally, we break the packet into any relevant fields (destination IP address/port, HTTP method, if applicable, and \etc) and save it in JSON format. Any PII found is redacted before saving the packet to allow us to share the data with the community. Any contextual information (the PII found, along with the application name, and whether or not this application was in the foreground when it generated the packet) is saved in separate JSON fields. Note that although the entire packet is not necessary for the purposes of this paper, the data could be useful later, for instance to train classifiers that predict PII exposures as in \cite{recon15} and \cite{antshield-arxiv}.

In summary, using \antShield to capture packets on the device has several advantages compared to previous datasets collected in the middle of the network: (1) we are able to accurately map each packet to the app that generated it; (2) we can keep track of foreground vs. background apps, to see what kind of data apps send while in the background; (3) we gain insight into TLS, UDP, and regular TCP traffic, in addition to HTTP and HTTPS; (4) scrubbing PII and labeling packets with the type of PII they contain is fully automated. Due to these advantages, we were able to collect comprehensive and realistic cases of PII exposures, as described in the next section.


%A key insight of our design is the distinction on whether PII of interest is known to the device or not. We refer to PII that consists of strings known a priori on the device (\eg via Android APIs, or defined by the user) as \preDefLeak . We refer to PII that is not known to our \antshield system (\eg hidden from apps or changing dynamically) as  \unknownLeak. By default, we assume that any PII available via Android API calls are \preDefLeak (\eg IMEI, AndroidID, phone number, serial number, ICCID, MAC Address, AdvertiserID, email, and location), and the rest are \unknownLeak (\eg username login, password, first/last name, gender, zipcode, and city). 


%{\bf What is a privacy leak?} Our system employs different techniques to detect the transmission of \preDefLeak PII (\stringMatch) and \unknownLeak PII (classification).
%
%We refer to the transmission of a packet from the device to the network, containing at least one  PII, as a {\em privacy exposure (or leak)}. This transmission may be: (i) intended to collect information about the user; (ii)  benign, \eg necessary for the operation of the app, acceptable to the user, or (iii)  of the honest-but-curious nature. Distinguishing between privacy {\em exposure} and an actual privacy {\em leak} is out of the scope of this paper, and we refer to the two terms interchangeably, meaning ``exposure.''  Our goal is twofold: (i) to present a system that detects privacy exposures
%
%{\em on the device} with low overhead, accurately and in real-time, and (ii) to design and analyze a user survey that captures what is considered a privacy leak via crowdsourcing.%, and raise the user's awareness.  % 
%This is a first step towards enabling distributed learning of PII exposures.

%{\bf Design Objectives and Choices.}  %
%
%
%First, we want a solution that can be used by the non-sophisticated end-user: a mobile app that the user can simply install (as an app, without rooting the phone), enable in the background, and occasionally interact with. Second, we want a solution that operates purely on the device and does not redirect traffic through a middle server. This has several advantages: it does not need to expand the trust base (data does not need to leave the user's device), and it is well positioned to have access to rich information available on the device  (app names, and \preDefLeak PII). To meet both of these goals, we use the  \antLib v0.1.5 \cite{antmonitor-arxiv}. To the best of our knowledge,   \anteater is the most efficient implementation (in terms of throughput, battery and other resources)  for on-device packet interception and inspection of both unencrypted and encrypted traffic, today; see \cite{antmonitor-arxiv} for details. \anteater relies on a VPN service on the device (but  not on a remote VPN server), which is the only way to intercept traffic today without rooting the phone.   If more efficient libraries for packet interception become available in the future, \antshield 's modular design allows to replace this component. 

%Third, we want to accurately detect a comprehensive range of PII in real-time, both \preDefLeak (through \stringMatch), and the remaining \unknownLeak ones through machine learning models. Towards the first goal, we utilize the DPI  API provided by \anteater \cite{antmonitor-arxiv}. %Towards the second goal, we build specialized classifiers defined in  Sec. \ref{sec:system-implementation}.

%
%\subsection{PrivacyShield Architecture} \label{sec:system-antShield}

 %The overview of the \antshield architecture is depicted in Fig. \ref{fig:antShield}. It consists of a mobile app and an (optional) server. A brief overview of each component is described next.

%{\bf Online Leak Detection.} %
%This is the core  functionality of our PII exposure detection. As shown in Fig. \ref{fig:antShield}, \antShield leverages calls to \antLib  ({\tt accept\-IP\-Datagram} and {\tt accept\-Decrypted\-SSL\-Packet})  to intercept packets (in clear text or decrypted SSL, respectively).
%Each outgoing intercepted packet  is analyzed with DPI for \preDefLeak leaks and for features. %The features are then passed to classifiers to detect \unknownLeak leaks (described in detail in Sec. \ref{sec:system-implementation}). Either way, if a PII exposure is detected, the user is notified and the exposure is logged. If the user chooses to, the leaky packet can be blocked, or it can be allowed to continue towards its remote destination. % 


%{\bf Offline Analysis.} This module can be used when heavier processing is required. %
 %For example, to generate logs on the device, which require I/O operations, we use \antLib's {\tt con\-sumePacket()} API from this module. This module can be used to generate ground truth on the device;  and in the future, it can be extended to re-train classifiers on the device without sending data to a central server. We used this core function to collect and label our datasets accordingly
%
%

%{\bf Storage (on-Device and/or Server).} The \antShield app comes pre-loaded with classifiers trained on our existing dataset (Sec. \ref{sec:data-ours}), so that users have no need to contact any server and can use the system as-is.  Only if the user chooses to  do so, logs (packet traces, JSON or other meta data) can be maintained on the device and/or occasionally be uploaded to a server. The use of the server is optional -- by default, logs do not need be collected or leave the device. The user may choose to share her data with the server to get the benefits of crowdsourcing, and retrained classifiers. As an example scenario, we used the logging capability of the Offline Analysis module to generate the dataset used in our evaluation. Specifically, each captured packet was labeled with the type of PII that it was leaking and the app name that generated the packet. The PII itself was replaced, and the packet was converted to a JSON format for easier processing at the machine learning training stage (see Sec. \ref{sec:data-ours} for details). In general, this feature is useful for other researchers  who may wish to generate their own datasets manually or from user studies.
  
 

%

%{\bf GUI.} This component has two purposes. It allows the user to specify various preferences,
% most importantly, the \preDefLeak PII to be monitored. By default, these include PII available on the device through Android APIs, as shown in Fig.  \ref{fig:guiPI}.  Users that trust \antShield can also opt-in and predefine additional PII, such as  name and gender or any string (\eg digits of a credit card). Second,  \antshield's GUI notifies the user about PII exposed. From here, users can decide to allow the leak to happen, replace the exposed PII with a random string of the same length (so as not to alter the payload size), or block the packet completely. Whatever action the user selects, it is remembered for future occurrences of the same PII/app combination. Users can view a history of leaks at any time and can also see where each app sends data as a graph of connections updated in real-time (Fig. \ref{fig:guiVisual}). The edges of the graph can be filtered or annotated by the leaked PII, and more information about the remote servers receiving the leak can be displayed.

%\subsection{Leak Detection Methodology}\label{sec:system-implementation} 


%At the heart of \antShield lies the online inspection of network packets to detect if they contain PII.

%First, we use a {\em hybrid} \stringMatch-classification methodology. As described in Sec. \ref{sec:problem-leak}, a key insight is that PII can be split  into two categories: \preDefLeak and \unknownLeak, depending on whether  they are known a priori or not. This is an inherent advantage of operating on the device: \antShield has access to all the \preDefLeak strings and can use DPI to search for them; we refer to this method as \stringMatch. This not only gives us 100\% accuracy on finding \preDefLeak leaks, if they are not obfuscated, but also reduces the set of PII that classifiers must learn, thereby improving the accuracy of finding \unknownLeak leaks and reducing variance (see Sec. \ref{sec:prediction-result}).

%Second, we treat PII detection as a \multiLabel problem, since a packet may contain zero, one, or multiple PII. Our classifiers decide,  in one step, if any PII are contained in a packet, and if so - what type. More specifically, we use Mulan \cite{mulan}  to perform multi-label classification using the Binary Relevance (BR) transformation method \cite{tsoumakas2006multi}. The idea is to train a separate binary classifier for each label. Since the C4.5 DTs worked well for classifying leak vs non-leak, we use them as the independent classifiers in BR. %

%Third, we build classifiers {\em per-app}, instead of {\em per destination domain}. This is possible thanks to   \antshield running on the device:  it can accurately map a packet to the app that generated it. From a classification point of view, per-app classifiers perform similarly to per-domain classifiers, as shown in Sec. \ref{sec:prediction-result} and explained in Sec. \ref{sec:findings}. However,  per-app classifiers have important system advantages. First, they allow for easy setup and scalability: only the few classifiers for the installed apps on the particular device must be loaded into memory. This is much smaller than hundreds of domains contacted by those apps and the third-party libraries contained within them. Second, they apply to all TCP and UDP traffic, not just to HTTP(S) traffic. Third,  per-app classifiers obviate the need for DNS lookups, which are costly and inaccurate, but are necessary when using per-domain classifiers. \recon parsed HTTP(S) packets to extract the host name (which is also costly in terms of CPU) and decided which per-domain classifier to apply. One possible solution is to do reverse-DNS lookup to map (all TCP and UDP, not only HTTP(S)) packets to their intended hosts. However, many companies opt-in to use third-party web service providers (such as Amazon AWS), and for them, reverse-DNS returns host names that are not very useful (\eg ec2-54-164-159-29.compute-1.amazonaws.com). As a \workaround, it may be possible to implement a reverse-DNS cache on the device by keeping track of all the DNS requests. Unfortunately, we have seen many cases where the same IP maps to multiple host names (again, due to third-party web service usage). Finally, even if we could somehow achieve perfect mapping of IPs to host names, there is still the problem of domain name extraction. One solution is to maintain a public suffix list, but that would take up too much memory on the mobile device. Another solution is to keep removing prefixes from the host name and do DNS queries until a Start of Authority record is reached; but this would cause too much network delay on each packet before it can even be assigned a classifier.



%\subsection{Real-time Implementation on the Mobile Device} \label{sec:opt}
%
%
%
%The classifiers described in the previous section have value on their own right. However, it is highly non-trivial to apply them in real-time on a mobile device, with limited CPU and RAM. \antshield is the first system to achieve this goal 
%
%thanks to the following system optimizations.

%{\bf Detecting PII in an Outgoing Packet.}
%
%
%Our hybrid approach relies on  \stringMatch to search for the \preDefLeak leaks and on classification methodology to detect \unknownLeak ones. The former benefits from the good performance of \antLib's efficient DPI module. The latter needs to parse packets to extract words that are used as features of the classifiers.  With off-the-shelf \recon, to extract words from a packet,  several invocations of Java string parsing methods would be required, which  are extremely slow on a mobile device. We were able to  extract features from the traffic while completely avoiding parsing by exploiting the following observation:  most decision trees are one-level deep and only a third of the trees have a depth greater than two. 
%Therefore, we only need to extract the words that appear in the decision tree nodes and we can use DPI to search for them. Since the Aho-Corasick algorithm used in the \antLib can search for many strings in one pass of the packet, having these extra words to  search for does not affect performance. 

%Extracting words that appear in the decision tree nodes and using DPI to search for them works well in most cases. However, in some cases the words are too small and can actually be part of a longer word. In this case, DPI search would mark a feature as existent, when in fact it's part of a different word, causing an incorrect prediction. As an example, {\em hulu} was receiving the word `\textvtt{profile}' in the packets that also contained the user's first name. However, many packets that did not contain any exposures, contained the word `\textvtt{video\_profile}.' To avoid these DPI-based false positives, we decided to keep the delimiters surrounding each word during feature selection. So, in the case of {\em hulu}, we used `\textvtt{/profile?}' as the feature. This trick allowed us to extract the same words with DPI as with Java parsing.

%{\bf Minimizing Classifiers to Load in RAM.} 
%
%With limited RAM, care must be taken when loading machine learning models from disk to memory. To minimize the impact on RAM, we: (i) load per-app models  only for those apps that are installed on the device; and (ii) perform a two-step training method to reduce the general classifier feature set (see Fig. \ref{fig:antShield}). Specifically, the general classifier has a feature set size of over 12k, and during prediction needs the  allocation of a double array with size 12k+. While this is a small size for a server, on the mobile device it causes major issues -- if one loads the full general classifier, most web pages and applications do not load. This is because each time a packet has to be predicted by the general classifier (when there is no corresponding per-app classifier), the memory allocation becomes so large that a {\em blocking garbage collection call} has to be executed by the Android OS after every prediction. This blocks the main networking thread, causes connections to time-out, and prevents pages from loading. We were able to reduce the feature set by exploiting the existing classifier tree: we re-trained the general classifier using only the words that appear in the tree nodes as features. This resulted in a feature set size of only 509, \ie  a 24x reduction for the general classifier, which in itself allowed \antShield  to run in real time. Further improvements were achieved by reducing the feature set of per-app classifiers. Overall, \antShield's memory usage was around 100 MB, which is acceptable: many  popular apps, \eg\xspace  {\em Facebook}, use as much as 200 MB RAM.


%{\bf Real-Time Packet-to-App Mapping.}
%
%In order to call the per-app classifiers, we first need to map a packet to the application that generated it. The \antLib provides packet-to-app mapping but only off-line (\eg after a packet has been read off a queue on a different thread that does not block the main networking thread) \cite{antmonitor-arxiv}, which is not fast enough to run on-line. Specifically, when using \antLib's original mapping implementation, we were only able to reach a throughput of 1 Mbps when testing with {\em Speedtest}. Upon further code and CPU usage analysis, we found that the inefficiency stemmed from two issues: (i) the \antLib was doing some Java string parsing to extract the app UID, source IP/port, and destination IP/port that were separated by a comma when returned from the native C module; (ii) the \antLib was storing the mappings in a HashMap keyed by a String (made of concatenating source/ destination IP/port numbers), which caused many String comparisons whenever an item needed to be fetched from the HashMap. To avoid these costly operations, we changed \antLib's native C module to return the app UID and the source port number only, as separate elements in an array. (it is best to avoid using complex data structures in native C). This way the Java part of the code could separate out the UID (and fetch the corresponding app name) and the source port of each open connection without doing any parsing. The source port number is then used as the key to the HashMap that fetches the corresponding app names. These improvements allowed us to do real-time packet-to-app mapping while achieving network speeds close to regular device operation speeds.

%{\bf Real-time.} The evaluation in Sec. \ref{sec:eval-time}  shows that our optimizations make the crucial difference for  being able to detect PII in real-time on the device: 1ms for extracting words (as opposed to 30ms+ if parsing out all words) and 1ms for classification.%

%\input{04-3-realtime}


==> exposures_exposed_soups21 arxiv-2/04-1-datasets.tex <==
%
\subsection{Datasets Collected} \label{sec:data-ours}

Using \antShield's packet capturing ability, we interacted with and collected packet traces from 400 most popular free Android apps, based on rankings in {\em AppAnnie} \cite{appannie}. We used a Nexus 6 device for our data collection, and
%We collected and analyzed two \antShield Datasets; Manual and Automatic. 
%We logged all packets generated by different apps on a test device (Nexus 6) and converted each packet into a JSON object that reported any PII exposures (see \ref{sec:problem-leak} for a list) and broke the packet into any relevant fields (destination IP address/port, HTTP method, if applicable, and etc).
collected two different datasets, depending on how we interacted with apps, as described next. \footnote{These datasets are publicly available at \cite{antmonitor-page}.}

{\bf Manual Testing.}  First, in order to capture PII exposures during typical user behavior, 
we tested the top 100 apps 
%most popular and free Android  apps, based on rankings in {\em AppAnnie} \cite{appannie}. %
in batches:  we installed 5 apps on the test device %
and then used \antShield to intercept and log packets while interacting with each app for 5min. 
%
After all apps in the batch were tested, we switched off the screen and waited 5min to catch  any packets  sent in the background. Next, we uninstalled each app %
and finally, turned off \antShield. 
%

{\bf Automatic Testing.} %
We also used the {\em UI/Application Exerciser Monkey} \cite{monkey} to automatically interact with apps.  This does not capture typical user behavior but enables extensive and stress testing of more apps. We  installed 4 batches of 100 applications each, and had {\em Monkey} perform 1,000 random actions in each tested app while \antShield logged the generated traffic. At the end of each batch, we switched off the screen of the test device and waited for 10min to catch additional exposures sent in the background. 

\begin{center}
	\begin{table}[t!]
		{\scriptsize
			\begin{tabular}[b]{|c|p{0.8cm} p{0.8cm}|} 
				\hline
				& \textbf{Auto} &  \textbf{Manual}\\[0.5ex] 
				\hline
				\# of Apps &414 & 149\\
				\hline
				\# of packets  &  21887 & 25189\\
				\hline
				\# of destination domains & 597 & 379\\
				\hline
				\# of exposures detected & 4760 &3819\\
				\hline
				\# of exposures in encrypted traffic & 1513 & 1526\\
				\hline		
				{\bf \# of background exposures} & 2289 & 639\\
				\hline
				\# of HTTP packets & 13694 &13648\\ 
				\hline
				\# of HTTPS packets &6830 &8103\\
				\hline
				{\bf \# of TCP packets} &867 &2264\\
				\hline
				{\bf \# of exposures in TCP (other ports)} & 38 &7\\
				\hline
				{\bf \# of UDP packets} & 496 &1174\\  
				\hline
				{\bf \# of exposures in UDP} & 17 &12\\ [1ex] 
				\hline
			\end{tabular}
		}
		\caption{Summary of Manual and Auto \antShield datasets collected on the device.}
		\label{tbl:summary}	
	\end{table}
\end{center}%\mbox{}

\begin{comment}
\begin{center}
	\begin{table}[t!]
		{\scriptsize
			\begin{tabular}[b]{|c|p{0.8cm} p{0.8cm}|p{0.8cm} p{0.8cm}|} 
				\hline
				&\textbf{ReCon Public dataset(s)}  &&   \textbf{\antshield dataset(s)} &\\[0.5ex]
				\hline\hline
				&\textbf{Auto} &  \textbf{Manual} & \textbf{Auto} &  \textbf{Manual}\\[0.5ex] 
				\hline
				\# of Apps & 564 & 91 &414 & 149\\
				\hline
				\# of packets & 16761 &13079 &  21887 & 25189\\
				\hline
				\# of destination domains & 450 &368 & 597 & 379\\
				\hline
				\# of exposures detected & 1566 & 1755  & 4760 &3819\\
				\hline
				%{\bf \# of \unknownLeak leaks} & 4 &78 & 483 & 516\\
				%\hline
				\# of exposures in encrypted traffic & - & - & 1513 & 1526\\
				\hline
				%\# of packets with {\bf multiple leaks} &50  & 224  & 1506 & 790\\
				%\hline
				
				{\bf \# of background exposures} & - & - & 2289 & 639\\
				\hline
				\# of HTTP packets & 16761 & 13079 & 13694 &13648\\ 
				\hline
				\# of HTTPS packets & - & -  &6830 &8103\\
				\hline
				{\bf \# of TCP packets} & - & - &867 &2264\\
				\hline
				{\bf \# of exposures in TCP (other ports)} & - & - & 38 &7\\
				\hline
				{\bf \# of UDP packets} & - & - & 496 &1174\\  
				\hline
				{\bf \# of exposures in UDP} & - & -  & 17 &12\\ [1ex] 
				\hline
			\end{tabular}
		}
		\caption{Summary of Datasets.  \recon is the previous state-of-the-art, collected in the middle of the network \cite{recon15}. \antShield's  Manual and Auto datasets were collected on the device.}
		\label{tbl:summary}	
	\end{table}
\end{center}%\mbox{}
\end{comment}

{\bf Summary.}  Since the two (Automatic and Manual)  \antShield Datasets capture different behaviors, we describe and analyze them separately. The  \antShield datasets are summarized in Table \ref{tbl:summary}. Other state-of-the-art datasets include \recon \cite{recon15} and \cite{Ren2018}. Our datasets confirm and extend the findings of previous work, as outlined in the next section. 
%next to the prior state-of-the-art PII datasets collected by \recon  \cite{recon15, Ren2018}. %
%Our resulting datasets contains more and richer information about exposures than before. Some  advantages are inherent to running on the device (\ie the ability to capture contextual information, including the app names). Other differences are due to changes in app versions and PII exposure  behavior over time. 
Thus, in addition to being used to 
%evaluate our methodology
generate survey questions in our user study (Sec. \ref{sec:user_study}), our datasets provide valuable insights on their own (Sec. \ref{sec:findings}), and we will make them available to the community.

==> exposures_exposed_soups21 arxiv-2/04-3-datafindings.tex <==
%
\subsection{PII Exposures Found in the Datasets} \label{sec:findings}

Our datasets provide us with insights into the current state of privacy exposures in the Android ecosystem. Some of the captured patterns were previously unknown, and are revealed for the first time here. 
For example, we were able to detect exposures happening in the background, exposures in plain TCP and UDP (not belonging to  HTTP(S) flows), 
%two orders of magnitude more  \unknownLeak leaks than before (which is crucial for training classifiers), several hundreds of packets with not one but multiple leaks  (which motivated our  \multiLabel approach), 
and malicious scanning for rooted devices.

\begin{comment}
\begin{table*}[t!]
	\centering
	{\scriptsize
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf \xspace App Name} & {\bf \xspace  Leak Type}  &  {\bf \xspace  \# Leaks \:}\\[0.5ex] 
			\hline
			\xspace com.roblox.client 2.280.107211 & \xspace Username, Location  &  \xspace 1234 \\
			
			\xspace com.ss.android.article.master3.2.7 & \xspace  \multirow{2}{*}{  \parbox{3.5cm}{City, Adid, Location, AndroidId, IMEI}}  & \xspace 766\\
			& & \\
			
			\xspace com.cleanmaster.security3.2.6  & \xspace Adid, AndroidId  & \xspace 511 \\
			
			\xspace com.cyberpony.stickman.warriors.epic1.3  & \xspace Adid, City, Location, Zipcode & \xspace 434 \\
			
			\xspace com.paypal.android.p2pmobile6.9.0 & \xspace \multirow{2}{*}{\parbox{3.5cm} {City, FirstName, LastName, SerialNumber, Zipcode, Adid, AndroidId, Password, Email}}  &\xspace 257 \\
			& & \\
			& & \\
			
		    \xspace com.weather.Weather7.7.1  &\xspace Adid, Location &\xspace 172 \\
		    
			\xspace com.pof.android3.45.2.1417399  &  \xspace Adid, Username, AndroidId &\xspace 136 \\
			
			\xspace com.bitmango.go.wordcookies1.1.9  & \xspace Adid, AndroidId  &\xspace 135 \\
			
			\xspace com.kiloo.subwaysurf1.68.0  & \xspace Adid, IMEI, AndroidId  &\xspace 101\\
			
			\xspace com.qisiemoji.inputmethod5.5.8.1570  &\xspace Adid, IMEI, AndroidId  & \xspace99 \\
			
			\xspace com.bitmango.go.blockhexapuzzle1.3.7  & \xspace Adid, AndroidId  &\xspace 97 \\
			
			\xspace com.bitmango.rolltheballunrollme1.6.5 & \xspace Adid, AndroidId  &\xspace 95 \\
			
			\xspace com.jb.zcamera2.48  &\xspace  \multirow{2}{*}{\parbox{3.5cm}{ Adid, AndroidId, IMEI, Email, IMSI}}  &\xspace 87 \\
			 & & \\
			
%
%
%
			\xspace $\cdots$ & \xspace $\cdots$ & \xspace $\cdots$ \\
			\hline
			\xspace All & \xspace All & \xspace 3819 \\[0.5ex] 
			\hline
		\end{tabular}
		\quad \quad
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf\xspace Domain Name} &  {\bf \xspace Leak Type}  & {\bf\xspace \# Leaks \:}\\[0.5ex] 
			\hline
			\xspace isnssdk.com & \xspace Adid, IMEI. AndroidId  &\xspace 739 \\
			\xspace roblox.com & \xspace Location &\xspace 679\\
			\xspace facebook.com & \xspace Adid  & \xspace651 \\
			\xspace rbxcdn.com  & \xspace Location  &\xspace 561 \\
			\xspace mopub.com & \xspace Adid  &\xspace 340 \\
			\xspace bitmango.com  &\xspace Adid &\xspace 262 \\
			\xspace paypal.com &  \xspace AndroidId &\xspace 257 \\
			\xspace appsflyer.com  & \xspace Adid, AndroidId  &\xspace 239 \\
			\xspace goforandroid.com  &\xspace Adid, IMEI, IMSI, AndroidId & \xspace 171 \\
			\xspace applovin.com & \xspace Adid & \xspace 157\\
			\xspace pof.com  & \xspace Adid, AndroidId  & \xspace 121 \\
			\xspace adjust.com & \xspace Adid  & \xspace 96 \\
			\xspace adkmob.com  &\xspace Adid, AndroidId  &\xspace 88 \\
			\xspace pandora.com   & \xspace Adid, AndroidId, Zipcode  & \xspace 78 \\
			\xspace wish.com  & \xspace Adid  &\xspace 78 \\		
			\xspace lyft.com & \xspace Location  &\xspace 68\\			  			  
			\xspace $\cdots$ & \xspace $\cdots$ & \xspace $\cdots$ \\
			\hline
			\xspace All & \xspace All & \xspace 3819 \\[0.5ex] 
			\hline
		\end{tabular}
	}
	%
	\caption{Manual dataset: Summary of applications and domain names with most leaks and their leak types}
	%
	\label{tab:leaks}
\end{table*}


\begin{table*}[t!]
	\centering
	{\scriptsize
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf\xspace App Name} &  {\bf \xspace Leak Type}  & {\bf \xspace \# Leaks \: }\\[0.5ex] 
			\hline
			\xspace cmbinc12.mb32b5.98 &\xspace  \multirow{2}{*}{  \parbox{3.5cm}{City, Adid, Location, AndroidId, Zipcode}}  & \xspace 1326 \\
			& & \\
			\xspace com.kitkatandroid.keyboard3.9.9 &\xspace  \multirow{2}{*}{  \parbox{3.5cm}{Adid, , Location, AndroidId, SerialNumber}}  & \xspace 1046\\
			& & \\
			\xspace com.episodeinteractive.android.catalog5.61.1+g  &\xspace \multirow{2}{*}{  \parbox{3.5cm}{ \xspace Adid, Gender, SerialNumber, AndroidId}}&\xspace 438 \\
			& & \\
			\xspace com.myyearbook.m11.8.0.681 & \xspace Adid, City, Location, Zipcode &\xspace 263 \\
			\xspace System0.1.5 &\xspace \multirow{2}{*}{\parbox{3.5cm}{ Username, City, Zipcode, Adid, AndroidId, Location, IMEI, IMSI}}  & \xspace 255 \\
			& & \\
			\xspace com.clearchannel.iheartradio.controller7.2.2  &\xspace Adid, Zipcode & 220 \\
			\xspace com.cmcm.live3.4.9  &\xspace \multirow{2}{*}{\parbox{3.5cm}{Adid, AndroidId, Location, IMEI, SerialNumber, IMSI}}  &\xspace 213 \\
			& & \\
			\xspace com.apalon.myclockfree2.29 &\xspace Adid, City &\xspace 206 \\
			\xspace com.freecraft.pocket.edition2.0  &\xspace Adid, City, Location, Zipcode  &\xspace 174 \\
			\xspace com.madebyappolis.spinrilla2.2.4  &\xspace \multirow{2}{*}{\parbox{3.5cm}{Adid, City, Location, AndroidId, Zipcode}} &\xspace 146\\
			& & \\
%
%
%
			\xspace $\cdots$ &\xspace $\cdots$ &\xspace $\cdots$ \\
			\hline
			\xspace All & \xspace All & \xspace 4760 \\[0.5ex] 
			\hline
		\end{tabular}
		\quad \quad
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf \xspace Domain Name} &  {\bf \xspace Leak Type}  & {\bf \xspace \# Leaks \: }\\[0.5ex] 
			\hline
			\xspace mopub.com & \xspace Adid  &\xspace 2878 \\
			\xspace pocketgems.com & \xspace AndroidId &\xspace 416\\
			\xspace applovin.com & \xspace Adid  &\xspace 409 \\
			\xspace appsflyer.com  & \xspace Adid  &\xspace 312 \\
			\xspace ksmobile.net & \xspace SerialNumber, Location, AndroidId  &\xspace 216 \\
			\xspace ihrhls.com  &\xspace Adid &\xspace 215 \\
			\xspace goforandroid.com &  \xspace AndroidId &\xspace 210 \\
			\xspace tapjoyads.com  &\xspace IMEI, AndroidId  &\xspace 169 \\
			\xspace amplitude.com & \xspace Adid &\xspace 152\\
			\xspace lkqd.net  & \xspace Adid, AndroidId  &\xspace 150 \\
			\xspace tapjoy.com & \xspace Adid, AndroidId  &\xspace 148 \\
			\xspace pinterest.com  &\xspace AndroidId  &\xspace 112 \\
			\xspace bitmango.com   & \xspace Adid  &\xspace 109 \\
			\xspace 3g.cn  & \xspace AndroidId  &\xspace 107 \\		
			\xspace instagram.com& \xspace Username  &\xspace 105\\	
			\xspace crashlytics.com  & \xspace Adid, AndroidId  &\xspace 98 \\		  			  
			\xspace $\cdots$ &\xspace $\cdots$ &\xspace $\cdots$ \\
			\hline
			\xspace All &\xspace All &\xspace 4760 \\[0.5ex] 
			\hline
		\end{tabular}
	}
	%
	\caption{Auto dataset: Summary of applications and domain names with most leaks and their leak types}
	%
	\label{tab:leaks2}
\end{table*}
\end{comment}



 \begin{figure}[t!]
	\begin{center}
		\subfigure[{\em Flow Free}, a puzzle game, exposes the user's city to an advertising server when the application is in the background]{\includegraphics[width=0.9\linewidth]{figs/com_bigduckgames_flow.pdf}\label{fig:bigduckgames}\hspace{6pt}}
		\subfigure[{\em MeetMe}, an app for meeting people on-line contacts different domains with different PII types depending on whether it is in the background or the foreground]{\hspace{6pt}\includegraphics[width=0.9\linewidth]{figs/com_myyearbook_m1.pdf}\label{fig:myyearbook}}
		%\vspace{-10pt}
		\caption{Application behavior exposing PII, while running in the background vs. toreground} %(building on top of \antLib v0.1.5).}%(a)(b) apply to all uses of the app. (c-f) are specific to Privacy Leaks.  (f) shows which apps send packets  to which IP destinations for all active connections and is updated in real-time.}%  \blind{A video and more details can be found on our website}%
		\label{fig:bg_exposures}
		%\vspace{-15pt}
	\end{center}   
\end{figure}

{\bf Background Exposures}. \antShield is in a unique position to capture exposures that happen in the background vs. foreground, and other contextual information that is only available on the device. Table \ref{tbl:summary} shows that there is a substantial number of background exposures (\eg half of all exposures in the automatic dataset) that should be brought to users' attention. % and be incorporated into learning algorithms.
%We observed an order of magnitude more background leaks in the top apps in the  automatic vs the manual datasets. One possible explanation is that the random clicks in the automated test lead to clicking on ads, which generate traffic even after the app moves to the background.  
Digging deeper, we found several interesting patterns in apps that expose PII both in the background and in the foreground. Fig. \ref{fig:bigduckgames} shows how {\em Flow Free}, a puzzle game behaves differently in the background vs. the foreground: in the foreground several device identifiers are sent to ad and analytics servers, and in the background, one of the ad servers (\textvtt{mopub.com}) also collects the user's city. Perhaps this information is needed to serve personalized ads based on the user's location, but it is unclear why it is needed when the application is in the background and no ads are being shown. Another example is {\em MeetMe}, an app for meeting people on-line, whose behavior is shown in Fig. \ref{fig:myyearbook}. In this case, the app collects less PII in the background, but is contacting more ad servers. Such findings are concerning, since apps are causing users data usage and are posing privacy risks even when the user is not interacting with the app.

%{\bf Auto vs. Manual}. Tables \ref{tab:leaks} and \ref{tab:leaks2} show the top apps/domains that collect the most PII in our manual and auto datasets, respectively. We find that the top apps and domains differ for each dataset, indicating that it is important to test apps manually so as to fairly represent what happens to real users. For instance, we see that the auto dataset is more ad-oriented, while the top domains for the manual dataset include non-ad networks such as \textvtt{facebook}, \textvtt{paypal}, and \textvtt{pandora}. This is most likely due to the fact that our {\em Monkey} tests ended up clicking on ads during the random events, whereas real users tend to avoid ads.

\begin{table*}[t!]
	\centering
	{\small
		%
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf App Name} &  {\bf Leak Types}  & {\bf Port}\\[0.5ex] 
			\hline
			\xspace System  &\xspace IMEI, IMSI, AndroidId &\xspace 8080 \\
			\xspace com.jb.gosms &\xspace  AndroidId  &\xspace 10086 \\
			\xspace com.jiubang.go.music &\xspace AndroidId &\xspace 10086 \\
			\xspace air.com.hypah.io.slither &\xspace Username  &\xspace 10086 \\
			\xspace com.jb.emoji.gokeyboard &\xspace AndroidId &\xspace 10086 \\
			\xspace com.gau.go.launcherex &\xspace AndroidId  &\xspace 10086 \\
			\xspace com.steam.photoeditor &\xspace AndroidId &\xspace 10086 \\
			\xspace com.jb.zcamera &\xspace AndroidId  &\xspace 10086\\
			\xspace com.flashlight.\-brightestflashlightpro &\xspace AndroidId &\xspace 10086\\[0.5ex] 
			\hline
		\end{tabular}
		\quad %\quad 
		%\vspace{5pt}
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf Domain Name} &  {\bf Leak Types}  & {\bf Port}\\[0.5ex] 
			\hline
			\xspace 206.191.155.105 &\xspace Username  &\xspace 454 \\
			\xspace 206.191.154.41 &\xspace Username &\xspace 454 \\
			\xspace 23.236.120.208 &\xspace AndroidId  &\xspace 10086 \\
			\xspace 3g.cn  &\xspace IMEI, IMSI, AndroidId &\xspace 8080 \\
			\xspace 23.236.120.220 &\xspace AndroidId & \xspace10086 \\[0.5ex] 
			\hline
		\end{tabular}
	}
	\caption{TCP packets (non HTTP/S) sending PII over ports other than 80, 443, 53}
	%
	\label{tab:tcp_leaks}
\end{table*}

{\bf Non-HTTP Exposures}.  Prior state-of-the-art datasets \cite{recon15, Ren2018}  reported only HTTP(S) exposures. Table \ref{tbl:summary} reports, for the first time, exposures in non-HTTP(S), including plain TCP or UDP packets. Our dataset contains 29 UDP exposures, all of which were exposing Advertiser ID and Location. As shown in Table \ref{tab:tcp_leaks}, we also found some apps (mostly games and photo-editing apps) that exposed the Android ID over non-standard (80, 443, 53) TCP ports, such as 8080 or 10086 (a port known to be used  by trojans, Syphillis and other threats \cite{portsguide}). The destination IPs could not be resolved by DNS, indicating that the application may have hard-coded those IPs. %We were also able to detect over 3000 TCP packets with PII exposure, most of which are TCP segments, belonging to a larger HTTP packet. It is important to be able to classify these packets as well, since we will be receiving them through the VPN during real time inspection in \antshield. 
%
%

\begin{table*}[t!]
	\centering
	{\scriptsize
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf \xspace App Name} &  {\bf \xspace PII Types}  & {\bf \xspace \# Exposures \:}\\
			\hline
			\xspace com.ss.android.article.master &\xspace  \multirow{2}{*}{  \parbox{3.5cm}{City, Adid, Location, AndroidId, IMEI}}  &\xspace 752 \\
			& & \\
			\xspace com.cleanmaster.security & \xspace Adid, AndroidId  &\xspace 174\\
			\xspace com.paypal.android.p2pmobile  &\xspace \multirow{2}{*}{  \parbox{3.5cm}{ City, FirstName, LastName, Zipcode, Adid, SerialNumber, AndroidId, Password, Email}}&\xspace 131 \\
			& & \\
			& & \\
			\xspace com.offerup&\xspace \multirow{2}{*}{\parbox{3.5cm} {Adid, Username, FirstName, Location, Zipcode, AndroidId} }  &\xspace 114 \\
			& & \\
			\xspace com.cmcm.live &\xspace \multirow{2}{*}{\parbox{3.5cm}{Adid, AndroidId, Location, IMEI, SerialNumber, IMSI}}  &\xspace 114 \\
			& & \\
			\xspace me.lyft.android &\xspace  \multirow{2}{*}{\parbox{3.5cm}{City, FirstName, LastName, SerialNumber, Zipcode, PhoneNumber, Location, AndroidId}}   &\xspace 112 \\
			& & \\
			& & \\
			\xspace com.pinterest  &\xspace Adid, AndroidId &\xspace 111 \\
			\xspace com.weather.Weather  & \xspace Adid, Location &\xspace 110 \\
			\xspace com.qisiemoji.inputmethod &\xspace Adid, IMEI, AndroidId &\xspace 83 \\
	  			  
			\xspace $\cdots$ &\xspace $\cdots$ &\xspace $\cdots$ \\
			\hline
			\xspace All &\xspace All &\xspace 3039 \\
			\hline
		\end{tabular}
		\quad \quad
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf\xspace Domain Name} &  {\bf \xspace Leak Types}  & {\bf\xspace \# Exposures \:}\\
			\hline
			\xspace mopub.com & \xspace Adid  &\xspace 2380 \\
			\xspace isnssdk & \xspace AndroidId, IMEI & \xspace805\\
			\xspace roblox.com  & \xspace Location  &\xspace 679 \\
			\xspace applovin.com & \xspace Adid  &\xspace 566 \\
			\xspace rbxcdn.com & \xspace Location  &\xspace 561 \\
			\xspace appsflyer.com  &\xspace Adid  &\xspace 549 \\
			\xspace facebook.com  & \xspace Adid  &\xspace 391 \\
			\xspace bitmango.com   & \xspace Adid  &\xspace 371 \\	
			\xspace goforandroid.com &  \xspace AndroidId &\xspace 262 \\	
			\xspace ihrhls.com  &\xspace Adid &\xspace 219 \\
			\xspace pocketgems.com  & \xspace AndroidId  &\xspace 211 \\
			\xspace ksmobile.net & \xspace SerialNumber, Location, AndroidId  &\xspace 159 \\
			\xspace tapjoy.com & \xspace Adid, AndroidId  &\xspace 151 \\
			\xspace tapjoyads.com  &\xspace IMEI, AndroidId  & \xspace147 \\
			\xspace wish.com & \xspace Adid &\xspace 139\\
			\xspace paypal.com  & \xspace AndroidId  &\xspace 131 \\		
			%\xspace pof.com& \xspace pof.com  &\xspace 122\\	
			
			\xspace $\cdots$ & \xspace $\cdots$ & \xspace $\cdots$ \\
			\hline
			\xspace All &\xspace All &\xspace 3039 \\
			\hline
		\end{tabular}
	}
	%
	\caption{{\small Summary of applications and domain names with HTTPS exposures in our dataset (manual and auto)}}
	%
	\label{tab:leaks_https}
\end{table*}

%
{\bf HTTPS Exposures}.
Since the usage of encryption is increasing, we also collected and analyzed PII sent over HTTPS.
%Due to their sensitive nature,  previous HTTPS datasets \cite{recon15} were not made publicly available and we had to collect our own. \blue{New Narseo's dataset?} 
Table \ref{tab:leaks_https} summarizes the exposures we discovered in HTTPS traffic. The top app \textvtt{com.ss.android.\-article.\-master} is a news app, thus it makes sense for it to query the user's city, perhaps to fetch localized news. However, it is unclear why the app needs the user's IMEI (when it already has the Advertiser ID) and the specific longitude and latitude coordinates of the user. In this case, the city is needed by the app, but the IMEI and location coordinates are potentially privacy exposures. Another example is \textvtt{com.cmcm.live} - it exposes 5 different device identifiers for no apparent reason. Hence, although well-behaving apps should use HTTPS, they should also be inspected for potential privacy exposures as not all information that they gather is necessary for their functionality. We also found that the majority of top domains receiving PII over HTTPS were ad-related. Although it is expected for ad domains to receive the Advertiser ID, other PII should not be collected. These findings motivated us to conduct the user study in Sec. \ref{sec:user_study} to crowdsource answers to the question of when a privacy exposure becomes a privacy leak.

\begin{table}[t!]
	\centering
	{\scriptsize
		\begin{tabular}{|p{2.5cm}|p{2cm}|p{2.2cm}|}
			\hline
			{\bf\xspace App Name} &  {\bf\xspace Domain}  & {\bf\xspace PII Types}\\
			\hline
			\xspace com.bitstrips.imoji 10.2.32, 10.3.76 &\xspace pushwoosh.com & AndroidId \\
			\xspace com.nianticlabs\-.pokemongo 0.57.4 &\xspace upsight-api.com  & Location, AndroidId \\
			\xspace com.psafe.msuite 3.11.6 , 3.11.8  & \xspace upsight-api.com & AndroidId \\
			\xspace com.yelp.android 9.5.1 &\xspace bugsnag.com  & AndroidId \\
			\xspace com.zeptolab.ctr.ads 2.8.0  &\xspace onesignal.com & AndroidId \\
			\xspace com.namcobandai\-games.pacmantournaments 6.3.0  &\xspace  namcowireless.com & AndroidId \\
			\xspace com.huuuge.casino.slots 2.3.185 &\xspace upsight-api.com & AndroidId \\
			\xspace com.cmplay.dancingline 1.1.1  &\xspace pushwoosh.com  & AndroidId\\
			\hline
		\end{tabular}
	}
	\caption{Applications with "jailbroken" field}
	%
	\label{tab:jaibroken_apps}
\end{table}

%

{\bf Checking for Rooted Devices}. We noticed a suspicious flag  called ``jailbroken'' or ``device.jail\-broken'' exposed by several apps (\eg com.bitstrips.imoji, com.yelp.android, \zeptolab, etc). This flag was found in the URI content or in the body of a POST method  in the packets, and it was set to  1 if the device was rooted, or to 0 otherwise. In Table \ref{tab:jaibroken_apps}, we show the applications that contain this field in our dataset and the domain to which the ``jailbroken'' flag is being sent. We also show other types of exposures that the particular domain collects. From the table, we see that the flag is usually accompanied with a device identifier. Several apps send this flag to the same domain (\textvtt{upsight-api.com},  an ad network), which indicates that an ad library is probably exposing this information, rather than the app itself.
%

\begin{figure*}[t!]
	\begin{center}
		\centering
		\includegraphics[width=0.99\textwidth]{figs/graph_leaks.jpg}
		\caption{Understanding the behavior of app that expose PII through graph analysis of the \antShield dataset. The graph consists of nodes corresponding to destination domains and edges  representing the similarity of two domains. Two domains are similar if there are common apps that send packets with PII exposures to both domains; the more common apps  expose PII to these domains, the more similar they are, the larger the width of an edge between them. The color of a domain node indicates the types of  PII it receives. One can observe from the graph structure that domains form communities that capture interesting patterns: (1) The large communities on the left and bottom consist mostly of ad networks; ad exchanges are nodes in between ad communities; (2) Facebook/Google domains are a different community on their own, on the top left; (3)  small apps contact only their own domain, leading to isolate domain nodes; (4) domains in the same community receive the same type of PII (as indicated by the color of nodes).}
		\label{fig:graph}
		\vspace{-15pt}
	\end{center}   
\end{figure*}



{\bf Behavioral Analysis of PII Exposures.}  An interesting direction for analyzing the \antShield dataset is via behavioral analysis. For instance, we can ask: (i) what can the communication between mobile apps and destination domains reveal about tracking and advertising? (ii) what type of information exposes to what domains and how to define similarity of apps or domains with respect to exposures? Fig. \ref{fig:graph}\footnote{This figure was first presented in Fig. 3 of \cite{antshield-arxiv} and is repeated here for completeness.} showcases one graph that visualizes similar destination domains with respect to exposures they received, as captured in the \antShield dataset.
%
We define  two domains to be similar if they are contacted by the same set of applications (see the box on the right inside Fig. \ref{fig:graph}).
%
For example, domains A and B are similar because they are contacted by two apps (app1, app2).
%
We depict the similarity of domains A and B as an edge on the graph of domains, at the bottom of the box.
%
This data can be readily extracted from our trace, together with the type of information that was transmitted from apps to domains.
%


The graph depicted on the left side of Fig. \ref{fig:graph} shows a projection of the underlying bipartite graph (middle step in the box) on domains (last step in the box); the graph is plotted  and analyzed using Gephi \cite{bastian2009gephi}. Nodes in this graph represent domains; the edges indicate similar nodes as per above definition; the width of the edge indicates the number of common applications; and the domain color corresponds to the type of exposed PII. The clusters of domains in the graph are the output of a community detection algorithm, which is a heuristic that tries to optimize modularity.\footnote{The main idea is that for specific node $i$, it tries to assign different communities of its neighbors like node $j$'s community as $i$'s community and compute the gain of modularity for whole network. The community which maximize the modularity will be the proper one. If the gain of modularity be negative or zero, $i$ keeps its community. This process is an iterative process which is done for all nodes. This algorithm is implemented in Gephi software \cite{bastian2009gephi}, and works with weighted graphs also.}

%
%The graph in Fig. \ref{fig:graph}  reveals  interesting patterns about PII exposures in the \antShield dataset.
%
Interesting patterns are revealed in Fig. \ref{fig:graph}. First, advertising is the result of coordinated behavior.
%
For example, it is easy to identify ad exchanges: \textvtt{mopub.com} is in the center of all communication; and \textvtt{inner-active.mobi} and \textvtt{nexage.com} are also clearly shown as hubs.
%
All three large communities on the bottom and left of the graph correspond to ad networks.
%
Second, on the top left, there is a community of domains that belong mostly to Google and Facebook, and two domains (\textvtt{pof.com} and \textvtt{plentyoffish.com}) of a dating service.
%
The latter could be because the dating app also sends statistics (\eg for advertising purposes) to Google and Facebook, in addition to its own servers, as suggested by the type of PII being sent (gender and device ID, represented by the yellow color).
%
Third, not all domains belong to a community: some are well-behaved and are contacted only by their own app.
%
For instance the white-colored domain \textvtt{zillow.com} towards the bottom center of the graph is an isolate node and only receives information about the user's location, which makes sense since it provides a real-estate service.
%
Another example is the blue-colored domain \textvtt{hbonow.com}: it is only contacted by its own app and only receives the Advertiser ID to serve ads.
%
Another observation from Figure \ref{fig:graph} is that most domains in the same community receive the same type of PII (as indicated by the domain color).
%
This can be explained by the common ad libraries shared among different apps that fetch the same PII.
%

In general, similarity of apps and domains based on their PII exposure found in their network activity can be exploited to detect and prevent abusive behavior (\eg advertising, tracking, or malware) in mobile traffic. This is one promising direction for future work.
%





==> exposures_exposed_soups21 arxiv-2/04-user_study.tex <==
%\section{Crowdsourcing privacy notion/ User study on Mobile Data Privacy} \label{sec:user_study}

\section{User Study: Mobile Data Privacy in Context} \label{sec:user_study}


In this section, we design a user study on Amazon Mechanical Turk (MTurk) in order to assess user's awareness and understanding of mobile data exposure, as well as their level of concern and potential for adopting solutions. We use the datasets collected in the measurement study in the previous section to present participants with real-world scenarios of private information that was actually exposed by mobile apps in our experiments. We present the user with information about the types of PII exposed,  as we as information about the {\em context} this exposure occured, \ie whether the PII  is shared with the application or a third party server;  what was the app category/intended functionality; whether it is shared in clear or encrypted text, etc.   We then ask the users to assess the legitimacy (\ie  whether the information is needed for the app's functionality) and the risk posed by the particular PII type exposed in that particular context. 
We also educate the participants on how a single piece of PII can lead to even more information being discovered when combined with data fetched from a data broker. Finally, we ask users before and after the survey whether they would use privacy enhancing tools. To the best of our knowledge, this user study is the first one that collects and analyzes user input in such fine granularity (context)  and on actual (not just potential or permitted) privacy exposures at large scale (as found in the packet traces of the measurement study).
%
%Using the dataset discussed in the previous section, we ran a user study to help us distinguish privacy leaks from privacy exposures and to learn how much users understand about privacy in the mobile space. In this section we present our user study: the questions we asked and workers' demographics 
%
Section \ref{sec:study_design} presents the design rationale and questions asked in the MTurk study.  Section \ref{sec:study_results} summarizes and analyzes the responses from \numUsers participants. 
%Our user study on AMT provides insight into how many of the collected privacy exposures are actually leaks, i.e. illegitimate exposures that are not needed for the app?s functionality. These insights are a first step towards understanding user interaction with fine-grained privacy preserving tools such as AntMonitor.

\subsection{User Study Design} \label{sec:study_design}

{\bf MTurk Setup.\footnote{We went through the IRB process in our institution and obtained exempt research registration HS\# 2018-4272  ``Amazon Mechanical Turk Survey on Mobile Data Privacy''}.} We designed a Human Intelligence Task (HIT) on Amazon Mechanical Turk (MTurk) \cite{mturk}
%,  where we recruited real users to help us understand how much they care about privacy and how comfortable they are with sharing certain mobile data with third party servers. Our target population consisted of 
and restricted it to workers who are based in the U.S., are at least 18 years old, have completed at least High School (in the US), and own a smartphone or a tablet device. %No personal identifiable information was collected during this study.
Our study was approved by the Institutional Review Board (IRB) of our Institution (details are omitted from this double-blind version). %\footnote{%IRB details:  04-26-2018  MOD 23912  HS\# 2018-4272}. 
The workers were rewarded at a rate of \$0.10 per minute of their time -- a standard followed in other studies \cite{Lin2012, Ismail2017, Mason2010}. We allotted 30 minutes for the completion of our HIT, but the majority of workers completed it within 13 minutes approximately. The participants had to pass at least one of three attention check questions in order to have their HIT approved and to receive the \$3.00 payment.
%The anwers of each worker were automatically approved after three days of each HIT completion. If the participants passed at least one of our three checks they were paid \$3.00 for a 30-minute HIT.
 The HIT was open for 9 days in early May 2018. %from May 4th 2018 5pm PDT until Sat. May 12th 2018 10pm PDT. 
 At the end, we analyzed the responses of \numUsers workers that passed the attention test.


{\bf Demographic questions.} First, we asked a set of demographic questions, such as educational level, age, and employment sector (tech vs. non-tech). We also asked what kind of mobile OS they use and how many different apps they use daily.  In addition to these questions, we added three attention-check questions to prevent workers from gaming the system by providing answers randomly. We discard answers from participants that failed to correctly answer all three attention check questions. %and/or provided incomplete answers in the categorization questions.


\begin{figure*}[t!]
	\begin{center}
		%
		\subfigure[Definitions used to categorize a PII exposure.]{\includegraphics[width=0.85\textwidth]{figs/survey_table_1a}\label{fig:survey_table_categories}}
		
		\subfigure[Definitions used to describe additional context of a PII exposure.]{\includegraphics[width=0.85\textwidth]{figs/survey_table_1b}\label{fig:survey_table_terms}}
		
%			\vspace{-10pt}
%		\includegraphics[width=8.5cm]{figs/informative_tables_merged}\hspace{6pt}
		\caption{Terms defined before being used in the categorization tasks.} 
		\label{fig:informative_tables}
		%	\vspace{-15pt}
	\end{center}   
\end{figure*}


{\bf Categorization questions.} The main goal of our study is to learn how concerned are users about privacy exposures in different contexts, defined as: the type of PII exposed, the app category, whether the information was shared with a relevant application server (thus may be useful for the functionality of the app) or third party advertiser and analytics servers, and whether it is shared in plain text or is encrypted. %
%%% This text is replicated in the tables"
%\begin{itemize}
%	\item Needed by the App (a privacy exposure). Example: location being sent to {\em Google Maps}.
%	\item Not Needed by the App, but not Harmful (a privacy exposure). Example: ads \& analytics servers collecting Advertiser IDs.
%	\item Not Needed by the App, and may be Harmful (a privacy leak). Example: phone number being sent by a music app to a remote server.
%\end{itemize}
To that end, we first defined these terms and categories as shown in Fig. \ref{fig:informative_tables}.  
%We provided users with definitions and examples for each category, as shown in Fig. \ref{fig:survey_table_categories}. In addition, we provided them with definitions of terms that are needed in order to make more informed decisions when categorizing exposures (Fig. \ref{fig:survey_table_terms}).
%
%To educate the participants about privacy on mobile phones, we present first two informative tables that show different types of information that might leak from mobile phones and what is considered harmful and what is needed for the functionality of an app. These tables, as shown in Fig. \ref{fig:informative_tables}, are essential for the categorization questions. In our study we have two types of categorization questions. 

%The first categorization task is about how comfortable they are with sharing certain information types with certain destinations. In particular, we asked the participants to consider different types of information available on their phone and shared by mobile apps with various servers and label accordingly each case with how concered they are with sharing a type of information with a certain destination. 
First, we asked the participants how comfortable they are with sharing various {\bf PII types} with different types of {\bf remote servers}, as depicted in Fig. \ref{fig:question_10}. Different PII types include: various device ids (such as phone number, IMEI, IMSI, ICCID, Android Id, etc), user ids (\eg email, Advertiser Id, username and password), location (GPS coordinates), and demographic information (\eg gender, city, zipcode, first and last name). Destination servers are roughly divided into two categories: app developers vs. ad \& analytics servers. The rationale is that the application servers may need the PII to perform their functionality (\eg\xspace {\em Google Maps} clearly needs location) while third party servers do not (thus causing more of a privacy leak rather than an exposure).  For each pair of (PII type, destination type) we asked the participants to rate their comfort level of sharing that PII type with that remote  server, on a scale from 0 to 3;  where 0 represents the least concern and 3 represents maximum concern (and their willingness to pay for a privacy-preserving solution). See Fig. \ref{fig:question_10} for details.
%In Fig. \ref{fig:question_10}, the exact question is shown along with the options the participants have.

 \begin{figure*}[t!]
	\begin{center}
		%

		\includegraphics[width=0.8\linewidth]{figs/question10_v2}\hspace{6pt}
		%
		%	\vspace{-10pt}
		\caption{Task to assess how comfortable users are with sharing certain {\bf PII type} with certain type of {\bf remote server}.} 
		\label{fig:question_10}
		%	\vspace{-15pt}
	\end{center}   
\end{figure*}



%36 total
Second, we asked participants to rate their concern in real-case scenarios of PII exposures from our dataset (Sec. \ref{sec:data}). For each packet that contained a PII in our dataset, we considered a {\bf broader context} beyond just {\em PII type} and {\em destination server type} (\ie application server or ad/analytics server). We also considered the category of the app (\eg game vs navigation), whether the PII was {\em encrypted} or sent in plain text, and the {\em  frequency} of this PII being exposed by this app category.  The rationale is that the same PII type exposed may be more or less concerning to users depending on the context. For example, location exposed by a navigation app to that app's server in an encrypted packet is probably needed for the app to function, while sending a user id to an unrelated third party (\eg advertiser) server, frequently and/or in plain text, is indeed a privacy leak. 


 \begin{figure}[t!]
	\begin{center}
		%
		%	\includegraphics[width=17.5cm]{figs/roblox_game_categ_merged}

		\subfigure[Warm-up question with a hypothetical scenario of a particular example application -- the game {\em Roblox}.]{\hspace{6pt}\includegraphics[width=0.99\linewidth]{figs/roblox_v3}\label{fig:roblox_v2}}
		\subfigure[Entire game category with real cases of PII types exposed and their broader context (remote  server type but also app category,  encrypted/plain text, and frequency).]{\hspace{6pt}\includegraphics[width=0.99\linewidth]{figs/game_categorization_v2}\label{fig:game_categorization}}
		%\subfigure[Categorization question for the Game category; a real-case scenario.]{\hspace{6pt}\includegraphics[width=8.5cm]{figs/game_categorization.png}\label{fig:game_categorization}}
		%
		%	\vspace{-10pt}
		\caption{Task to assess user concern about {\bf privacy exposures in context.} }
		\label{fig:categorization_questions_game}
		%	\vspace{-15pt}
	\end{center}   
\end{figure}

A side benefit of the aforementioned categorization is that it helped reduce the number of cases to be evaluated by users. Out of 8,579 exposures total (Table \ref{tbl:summary}), 1,726 are unique when considering the application responsible, the type of PII, the destination host, and level of encryption. To further reduce the number of cases to label, we grouped the applications based on their {\em Google Play Store} \cite{googleplay} category and destination type (ad \& analytics or not). To find ad \& analytics domains, we used the {\em hpHost} \cite{hphosts} list as it was found to be the most comprehensive list for the mobile ecosystem to date \cite{vallina2018tracking}. These grouping reduced the total number of unique combinations to 256, which contained 23 unique {\em Google Play Store} categories (out of 36 total). We split these combinations into five batches of HITs, where each HIT contains five (or three for the last batch) categories of apps to be labeled.
%In the second categorization task, we asked the participants to categorize a set of real-case scenarios that consisted of a certain app category, as defined in Google Play, and the PII leaks that we extracted from our datasets by grouping the tested apps into the aforementioned categories. In particular, we showed them 23 different categories of apps and their according information types that are destined to either Analytics/Ads servers or App Developer servers. For this kind of categorization task, the participants must take into consideration each information type, its destination, whether it is encrypted, and how frequently it is being shared with the according destination (Advertisers or App Developer). 
To prepare the participants for the labeling task, we first showed a ``warm up'' question (Fig. \ref{fig:roblox_v2}) with a hypothetical scenario of the {\em Roblox} app exposing certain PII and asked them to assess the risk (Fig. \ref{fig:survey_table_categories}). Next, we asked the participants to label the exposure scenarios for each of the five categories in their HIT -- example shown in Fig. \ref{fig:game_categorization}. We also provide an example app out of each category (from our actual dataset) along with a link to the app's {\em Google Play Store} page.




%This question aims to prepare the workers for the real categorization questions, which are based on our real-case scenarios extracted from our datasets. We also demonstrate an example with the ``Game'' category (Fig. \ref{fig:categorization_questions_game}) , where the users must categorize each Information type to the according category.  In this case, the username might be necessary for a game, when it is destined to App Developer servers (in encrypted way) and the game asks the user to create an account before playing.  Another PII that leaks from the ``Game'' category is the Advertiser Id, with a high frequency and it is sent unencrypted to Ads servers. This can be considered as not needed by the App and not harmful, since it is needed by certain (free) games, that contain ads. On the other hand, the gender information might be considered a harmful leak, when it is sent to App Developer unencrypted, as it is not necessary for the app's functionality.

%Finally, we ask the workers to assess different scenarios of certain information type that is leaking from a certain category of apps. We splitted our 23 categories of apps and their PII leaks into five batches, where each HIT contains a batch of five (or three for the last batch) categories of apps to be labeled. We would like to highlight that the scenarios are based on our real dataset that we generated manually, that is we gathered apps that leak information and grouped them by category such as game, music \& audio etc. In order to facilitate user evaluation, we also provide examples of some real apps for each category and their links to Google Play \cite{googleplay}, as shown in Fig. \ref{fig:categorization_questions_game} in the right figure. 

\begin{figure}[t!]
	\begin{center}
		%
		\subfigure[How much do users care about privacy?]{\hspace{6pt}\includegraphics[width=0.8\linewidth]{figs/question_8.png}\label{fig:question_8}}
		\subfigure[How much would users pay to protect their privacy?]{\hspace{6pt}\includegraphics[width=0.8\linewidth]{figs/question_11.png}\label{fig:question_11}}
		\subfigure[Would users contribute their data to a privacy app?]{\hspace{6pt}\includegraphics[width=0.8\linewidth]{figs/question_12.png}\label{fig:question_12}}
		\subfigure[Do users care more after being educated about data brokers?]{\hspace{6pt}\includegraphics[width=0.99\linewidth]{figs/question_20v2}\label{fig:question_20}}
%		\subfigure[Follow up question about data contribution.]{\hspace{6pt} \includegraphics[width=7.5cm]{figs/question_21.png}\label{fig:question_21}}
		%
		%	\vspace{-10pt}
		\caption{Assessing users concern and potential actions. (a) Do users care about privacy?  What they are willing to do about it: (c) share their data with a crowdsourcing system (b) use and/or pay for a privacy app). And (d) do they change attitude after being educated?} 
		\label{fig:questions_how_much_they_care}
		%	\vspace{-15pt}
	\end{center}   
\end{figure}


{\bf Assessing User Concern and Possible Actions.}  In order to assess participants' privacy awareness and understanding, we asked another set of questions shown in Fig. \ref{fig:questions_how_much_they_care}. First, we asked the participants how much they care about information being shared by their mobile device (Fig. \ref{fig:question_8}) and what would they do in order to better protect their information. Next, we asked if they would use an app (\eg \anteater) that can prevent privacy exposures and how much would they pay for such a service (Fig. \ref{fig:question_11}). It was our hope that the categorization questions described previously would educate users about mobile privacy and would make them more concerned towards the end of the survey. To educate them further, we showed them that a single PII in the hands of a data broker can help create or lookup a user profile and can reveal much more information (Fig. \ref{fig:question_20}); the question was based on a real scenario where we fetched data from a data broker based on a person's email address. 
%To assess our hypothesis that users became more privacy-aware after the categorization questions and the data broker example,
%At the end of the survey, we showed them a real-case scenario after we entered a person's email in a data broker website.  We demonstrate what information that was known about this person, as shown in Fig. \ref{fig:question_20}. This information is likely to be shared across different data brokers and ad exchange services in order to provide targeted ads to this person for money in exchange. Next, 
We then asked them (if they would use a privacy app 
%after knowing this information can be known by data brokers 
(and if they would pay for it) to protect their privacy. %, in order to observe if the users become more privacy-aware at the end of they survey.
Finally, we asked them if they would contribute their mobile data to an app that crowdsources information, train machine learning models and prevents privacy leaks (\eg as in \recon \cite{recon15} and in \cite{antshield-arxiv}). %after showing them what information can be known about a person to data brokers by only providing their email address (Fig. \ref{fig:question_20}). The reasoning behind this question was 
In order to assess our hypothesis that users became more privacy-aware after the categorization questions and the data broker example, the same questions appeared twice during the survey: once in the middle of the survey and once at the end.






\subsection{User Study Results} \label{sec:study_results}

In this section, we summarize and analyze the main results of our user study. The main observation is that users seem initially confused about the severity of PII shared in different contexts, but they are interested in and are capable of being trained. Our main findings are as follows:

	\begin{itemize}
		\item Users do not seem to understand how severe it is to share certain PII types (especially device identifiers) with either Advertisers or Developers. This may be because some of these ids, such as Android ID, IMEI, IMSI, ICCID, are difficult to understand or relate to, yet they uniquely identify the device and/or the user and hence should not be shared with remote servers. % When they are shared in unencrypted manner this is even more severe and it considered a bad practice.
		\item As expected, users trust Application Developers more than Advertisers \& Analytics. However, some comments stated that Developers are ``a bunch of hackers behind servers,'' indicating possible confusion.
		%The opposite is true: application servers may actually use some of the information to provide a service (\eg location is needed by Google Maps), while sharing PII with advertisers has no functional role.
		\item Users also seem confused about sharing PII in plain text vs. using encryption. %Devices identifiers should not be shared with any destination even when they are encrypted. Location data are needed by certain app categories, but when they are shared unencrypted this is considered a bad practice. The same applies to username when shared unencrypted, since anyone that is sniffing into the network can access them. 
		Sharing PII in plain text is a bad practice, since it exposes private information not only to the destination servers but also to anyone that is sniffing into the network.
		\item Towards the end of the study, most users seem to obtain a much better understanding of mobile privacy. For example, several comments state that users are grateful for our short tutorial in mobile privacy. They are willing to educate themselves more in the future and to adopt data transparency and privacy tools. These are encouraging results for future work in developing privacy-enhancing technologies.
	\end{itemize}


\subsubsection{Summary and Demographic Info.} %\magenta{[Titles, order and styles here should be consistent with titles in Design Section.]}
%{\bf User demographics.} 
We collected 223 responses, in total,  on our MTurk survey. Since we posted multiple HITs, each with different categorization questions (see Sec. \ref{sec:study_design}), some users completed more than one HIT, and there were a total of 151 unique participants. Two responses were discarded due to failing the attention-check questions, and one worker was discarded due to incomplete answers. This leaves a total of \numUsers valid responses, which we analyze in the rest of the section. 
%
The majority of the participants were between 25 and 34 years old, held a Bachelor's degree and were employed in a non-tech sector. 61.8\% and 37.7\% of the workers were Android users, and iOS users, respectively. 118 of our workers use six to ten different apps every day, 53 use between 11 and 20 apps, 41 use fewer than five apps, and only 8 use more than 20 apps.

% Stats:
%6-10: 53.6%, 0-5: 18.6%, 31+: 1.8%, 11-20: 24%, 21-30: 1.8%


%{\bf Data Contribution.} We asked the participants if they are comfortable with sharing their data with a privacy app in order to improve its machine learning algorithms. In Fig. \ref{fig:all_data_contribution_before_after} , we demonstrate the collected answers from the beginning of the user study and the answers we collected from the end of the study, after we educated the users about privacy. We observe that users became more open to sharing their data with an app that protects privacy and aims to improve privacy leaks prediction. In particular, more users are willing to share their data for free in order to improve an app that protects their private information from leaking. On the other hand, the number of users that deny sharing their data is stable and it does not change towards the end of the study. Moreover, the number of undecided people is slightly decreased at the end of the study, as the partipicants become more aware about privacy risks.

%\subsection{Categorization results: What to protect and what not to protect?}
\subsubsection{Categorization Results: Privacy Exposures in Context.}

In this subsection, we provide the results we obtained by processing user answers to the categorization questions (see Figures \ref{fig:question_10} and \ref{fig:categorization_questions_game}). We asked participants to rank the severity of PII exposures in different contexts since whether or not an exposure is considered a privacy leak depends on the context. There are four main dimensions in each exposure: (i) its destination (app developers or advertisers), (ii) category of the app responsible, (iii) level of encryption used, (iv) PII type. These dimensions play an important role in distinguishing privacy leaks from exposures. 
%\magenta{[Talk about Context, leak vs exposure]}  


\begin{figure*}[t!]
	
	\subfigure[Rated by users]{\hspace{6pt}\includegraphics[width=0.2\linewidth]{figs/heatmap_sharing_all_workers.png}\label{fig:comfort_to_share}}
	\subfigure[Rated by us]{\hspace{6pt}\includegraphics[width=0.45\linewidth]{figs/ideal_heatmap_sharing_with_color_legends.pdf}\label{fig:ideal_heatmap_comfort}}
	\caption{How comfortable are users with sharing PII with advertisers and app developers? (a) Average rating of user responses to categorization task  of Fig. \ref{fig:question_10} (b) Recommended rating by us (``experts''). }
		\label{fig:heatmap2}
	\vspace{-15pt}
\end{figure*}

Figure \ref{fig:comfort_to_share} demonstrates the results when we asked the users how concerned they are with sharing a certain information type with a particular destination (Advertisers \& Analytics or App Developer servers), as shown previously in Fig. \ref{fig:question_10}. In this task, we observe that sharing all types of PII is concerning for our participants, regardless of its destination, and they are willing to use a free app to protect them. Furthermore, they would also pay for a tool that protects their phone number and password from leaking to advertisers.
%Moreover, device identifiers are also considered worth protecting for a price, especially when they are destined to advertisers. 
As expected, participants are more concerned over their precise longitude and latitude coordinates being shared as opposed to zipcode and city.
%However, password seems to be more important to block from advertisers and less important to protect from app developer servers, which can be true if an app requires login. 
Overall, our participants seem to trust developers more than advertisers, which is not surprising. 

In Fig. \ref{fig:ideal_heatmap_comfort}, we also provide our own ``expert'' rating for comparison. In particular, we would like to protect device identifiers regardless of their destination, by using a paid solution if a free version is not available. In contrast, our participants chose only to protect their device identifiers with a free solution and they are not willing to pay to protect them. Moreover, they give similar rating to their location data regardless of the destination, although they should be more careful with advertisers than developers, as there are apps that need location in order to function. On the other hand, Advertiser ID should not be protected as well as the other identifiers, since this id is known by advertisers anyway. 

{\bf Understanding whether PII is needed by the app.}
We ask users to assess whether sharing a particular PII is legitimate and needed for the functionality of the app (or more broadly by apps in the same category), or if it is unnecessary and potentially harmful. For example, GoogleMaps is an app in the Navigation category and needs to share location to provide the service.

 \begin{figure*}[t!]
	\begin{center}
		%
		%\vspace{-10pt}
		%\includegraphics[Average user ratings (left) vs. recommended rating by us (right)]{\hspace{6pt}
		\includegraphics[width=0.85\linewidth]{figs/heatmap_merged_leak_level.pdf}
%	\label{fig:heatmap_legitimate_non_legitimate}\hspace{6pt}}
		%\subfigure[Ideal merged heatmap]{\hspace{6pt}\includegraphics[width=5.5cm]{figs/our_heatmap_noted}\label{fig:our_heatmap_noted}\hspace{6pt}}
		\caption{Heatmap severity of (PII type, app category). The darkness of the color indicates the perceived severity of the PII exposure: the darkest corresponds to 4.0 (``Not needed by the app and maybe harmful''), while the lightest indicates 1.0 (``I don't care''). Zeros represent missing values for combinations we did not have in our datasets. We compare the average ratings among users who answered that question (on the left column) vs. labeling recommended by us (on the right column).}%Heatmaps of labeling information type as legitimate or not and how comfortable users are with sharing it with advertisers and app developers}
		\label{fig:heatmap_legitimate_non_legitimate}
		\vspace{-15pt}
	\end{center}   
\end{figure*}

Fig. \ref{fig:heatmap_legitimate_non_legitimate} presents a heatmap of the perceived severity of different PII types per application category. 
The x-axis show the different PII types and the y-axis contains the categories of apps responsible for sending that PII over the network. The values and colors represent the level of concern the participants have regarding each pair (category, PII type): ``not needed by the app and maybe harmful" (value 4 - dark color), ``not needed by the app and not harmful" (value 3), ``needed by the app" (value 2), ``don't care" (value 1 - light color). White color (or 0 value) represents missing combinations of PII and category, that were not present in our datasets. 
In order to produce the heatmap, we consider the mean values of all participants' answers. 

For comparison, we also show a heatmap labeled by us to express our ``expert'' opinion. First, location information (latitude and longitude coordinates, zipcode, and city) should be available to system, maps \& navigation, weather, and travel \& local categories only. All the other categories do not need this kind of information for their functionality and hence when apps transmit such data, it may be considered harmful. Second, user identifiers, such as email, password, username, gender, \etc may be needed in some app categories (\eg social, games, communication), but not in others (\eg photography, personalization, tools). Finally, device identifiers, such as IMEI, IMSI, Serial Number, ICCID, and Android ID should not be used by any app category, except perhaps for the System. These identifiers are unique and can be used to track users across different apps and build profiles, such as the one we showed in Fig \ref{fig:question_20}. Furthermore, Google explicitly discourages app developers from using these identifiers and asks them to instead create and use their own unique identifiers within their app \cite{googleids}. 

Comparing the two heatmaps in Fig. \ref{fig:heatmap_legitimate_non_legitimate} reveals that users are not as concerned about device identifiers as they should be: %most %\magenta{[be precise]} 
32.6\% of the device identifiers per app category were categorized by workers  as ``Not needed by the app and not harmful,'' although they should only be accessed by the System. However, other responses make sense: app categories that should not require any information to function are trusted the least (games, lifestyle, music \& audio, personalization, and tools), and categories such as weather and travel \& local are trusted with location information.



 \begin{figure*}[t!]
	\begin{center}
		\subfigure[Exposures in plain text: Avg user rating vs. our recommended rating]{\hspace{6pt}\includegraphics[width=0.55\linewidth]{figs/unencrypted_heatmaps_merged}\label{fig:heatmap_unencrypted}\hspace{6pt}}
		\subfigure[Exposures in encrypted traffic: average user rating]{\hspace{6pt}\includegraphics[width=0.35\linewidth]{figs/encrypted_with_labels}\label{fig:heatmap_encrypted}\hspace{6pt}}
		%\subfigure[Encrypted - ideal]{\hspace{6pt}\includegraphics[width=5.5cm]{figs/ideal_heatmap_encrypted}\label{fig:ideal_heatmap_encrypted}\hspace{6pt}}
		%\subfigure[Unencrypted - ideal]{\hspace{6pt}\includegraphics[width=5.5cm]{figs/ideal_heatmap_unencrypted}\label{fig:ideal_heatmap_unencrypted}\hspace{6pt}}
		\caption{Heatmaps assessing the severity of exposures in encrypted vs. unencrypted packets, as assessed by users  vs. us (``experts'').} %\magenta{[scale should be 0,1,2,3,4, not 0.8!!]}}%Heatmaps of labeling information type as legitimate or not and how comfortable users are with sharing it with advertisers and app developers}
		\label{fig:heatmaps_encryption}
		\vspace{-15pt}
	\end{center}   
\end{figure*}

{\bf Understanding Encryption.} %Since our dataset and our questionnaire contained  contextual information regarding use of encryption and remote servers,
%We also distinguish these PII leaks into harmful and not harmful categories based on the encryption techniques and destinations. To do this, 
We further split the heatmap in  Fig. \ref{fig:heatmap_legitimate_non_legitimate} into  Fig. \ref{fig:heatmap_unencrypted} and Fig. \ref{fig:heatmap_encrypted}, depending on whether the unencrytetd packet containing the PII was unencrypted or encrypted, respectively. Our heatmaps not only reveal participants' opinions about exposures, but also showed behavioral patterns of app categories. From Fig. \ref{fig:heatmap_unencrypted}, we see that the weather category does not use encryption and sends Advertiser Id, Location and City to remote servers in plain text. Similarly, maps \& navigation category sends Serial Number, Location, Zipcode and City information in plain text, but encrypts the Android ID and Advertiser ID. Sending PII in plain text is more harmful since this traffic can be sniffed. Unfortunately, our MTurk participants did not seem to understand the implications of transmitting data in plain text.



\begin{figure}[t!]
	\begin{center}
		\subfigure[PII sent to Ad Servers.]{\hspace{6pt}\includegraphics[width=0.8\linewidth]{figs/advertisers_destination_heatmap}\label{fig:advertisers_destination_heatmap}\hspace{6pt}}
		\subfigure[PII sent to Developer Servers.]{\hspace{6pt}\includegraphics[width=0.99\linewidth]{figs/developer_heatmap_with_color_labels.pdf}\label{fig:developer_destination_heatmap}\hspace{6pt}}
		\caption{Heatmaps assessing the severity of PII sent to different destination: Third-party (Ad Servers) vs  App Developers. Assessed by users (average user rating shown). The darker the color the more concerned the users).}
	\end{center}
\end{figure}

{\bf Understanding Destinations.} We also split our heatmaps based on whether the packet is going to App Developers (Fig. \ref{fig:developer_destination_heatmap}) or Advertiser \& Analytics Servers (Fig. \ref{fig:advertisers_destination_heatmap}). As expected, developers require more types of information in contrast to advertisers. On the other hand, advertisers should ideally only require the Advertiser ID, which is indeed fetched by almost every app category. However, most of our participants indicated that none of the PII need to be sent to advertisers for the app's functionality (only 2 out of 31 values in Fig. \ref{fig:advertisers_destination_heatmap} are below 2.5). This indicates that perhaps users don't consider ads being served a part of the app's functionality. In contrast, participants indicated more trust towards app developers (Fig. \ref{fig:developer_destination_heatmap}), which is expected as certain app categories require PII to function correctly. For example, the following pairs of PII and categories are expected: username for applications with logins (communication, games, and social), email for communication, and location information for travel \& local and maps \& navigation. However, device identifies, such as IMEI, IMSI, Serial Number and Android Id are not needed by any app category and they should not be shared with advertisers nor developers. Our participants seem to not understand this point and they labeled most of these exposures as ``Not needed and not harmful,'' while in fact these ids are most likely used for tracking. One interesting finding is that participants showed more concern over their IMEI vs. other device identifiers. This indicates that they may need more education about the other device identifiers.

%By examining the PII sent to  Developers (Fig. \ref{fig:developer_destination_heatmap})), we can see that most of this information \magenta{[specifics]} is required for an app category to function correctly. However, we would like to highlight that device identifiers should not be used by app developers in order to track the users, as this is considered a bad practice. Instead, they should create unique identifiers within their app and use these. Most \magenta{[precise numbers?]} seem to  understand these risks and they label only credentials like (password, username ) as useful for the app category.

\subsubsection{Towards A Solution: Tools Enhancing Data Transparency and Privacy.} %% Towadrs a Privacy-Preserving App. 

Fig. \ref{fig:question_8_ans_know_about_leaks} shows the distribution of answers to the questions of Fig. \ref{fig:questions_how_much_they_care}, which essentially ask how much users care about privacy exposures and what they are willing to do about it. The overwhelming majority of users would like more control over their information being shared, if a free option is available. Fig. \ref{fig:payment_before} demonstrates what payment options users would prefer for a privacy app: the majority would prefer a one-time fee between \$1 and \$5, than a subscription model. These results show that users are not only interested in using privacy-preserving tools  but are also willing to pay for them.
%, while a few of them would prefer to download once for less than \$1 and only of them would use a subscription of \$1 to \$5 per month.  However, the majority of the workers can pay for a privacy app if it is a one-time fee from \$1 to \$5. 
Towards the end of the study, after being educated about the extent and severity of  sharing PII, more users were willing to pay for a privacy app, \eg compare Fig. \ref{fig:question_8_ans_know_about_leaks} to Fig. \ref{fig:payment_after}. This demonstrates that although users may originally not be aware or understand the risks of privacy exposures, they become more weary after being educated about  the occurrence and risks of sharing PIIs (especially after learning the power of data brokers). 
%After presenting what information is available for data brokers, which is likely to be distributed to advertisers and analytics, we observe that most the participants would use a gree privacy app to protect such information. The number of workers that would pay for such an app is also significant. 
Finally, Fig. \ref{fig:all_data_contribution_before_after} shows the user's willingness to contribute data to a privacy-preserving tools that crowdsource information (such as \haystack, \recon, \anteater) before and after completing our survey. Once again, completing the study made users more open towards using and helping a privacy-preserving app. %\magenta{In summary, ...}

 \begin{figure}[t!]
	\begin{center}
		%
		\subfigure[How much users care about privacy exposures.]% \blue{Make titles consistent with question:DONE!}]
		{\hspace{6pt}\includegraphics[width=0.45\linewidth]{figs/question_8_ans_know_about_leaks.png}\label{fig:question_8_ans_know_about_leaks}}
		\subfigure[Monetization question at the beginning of the study.]{\hspace{6pt}\includegraphics[width=0.45\linewidth]{figs/all_payment_before.png}\label{fig:payment_before}}
		\subfigure[Monetization question at the end of the study.]{\hspace{6pt}\includegraphics[width=0.45\linewidth]{figs/all_payment_after.png}\label{fig:payment_after}}
		%	\subfigure[Data contribution answers from Master workers only]{\hspace{6pt}\includegraphics[width=3.5cm]{figs/data_contribution_before_after.png}\label{fig:data_contribution_before_after}}
		\subfigure[Data contribution in the beginning vs. at the end of study]{\hspace{6pt}\includegraphics[width=0.45\linewidth]{figs/all_data_contribution_before_after.png}\label{fig:all_data_contribution_before_after}}
		%
		%	\vspace{-10pt}
		\caption{Answers to questions of Fig.  \ref{fig:questions_how_much_they_care}: how much do users care about mobile privacy and what they are willing to do to protect it? Some  questions are purposely repeated in the beginning and at the end of the study.} 
		\label{fig:answers_how_much_they_care}
		%	\vspace{-15pt}
	\end{center}   
\end{figure}


\subsubsection{User Comments.}
%{\bf User comments/impressions.} 
At the end of the study, we asked participants for their comments and suggestions; 99 out of \numUsers users provided their feedback. In Fig. \ref{fig:comments}, we summarize the comments of all workers in the form of a wordcloud.
Overall, our \mturk workers seemed satisfied with the survey and stated that it was an educational experience. 
Most of the participants are thankful for our short tutorial on mobile privacy, as they gained more knowledge about privacy and how different apps share their information with various destinations. At the end of the survey, they seem more concerned about privacy and interested in a solution, including a privacy app free or paid; see Fig. \ref{fig:answers_how_much_they_care}.       %, while others would like this service to be available for free. 
Several participants mentioned the recent Facebook and Cambridge Analytica scandal and wondered if our user survey was inspired by it (it was not!). %Although this is not the case, we believe that this scandal was a wake-up call for many users of social media, however, mobile data privacy is also intrinsic nowadays. 
Below, we provide a sample of representative user comments, out of 99 total comments, grouped by two recurrent topics. 
%\magenta{[Out of how many total comments? Group by topic or frequency?]}

\begin{quote}
%\item \textit{``Maybe you should include what Facebook did involving a company called Cambridge Analytical, w involved fooling people to get their information. Like include questions that speak to the methods Cambridge Analytical used to steal people's identity/ fool people into to thinking they were  signing up for one thing but turns out it was for something else.''}

\item {\bf They learned a lot:}
\item \textit{``I liked this. Was this all due to what is going on with Facebook and other privacy	concerns?''}
\item \textit{``I enjoyed taking this survey.  I would not share my information with anyone that would use the information in anyway that would be damaging to my life.  Right now I am getting phone calls I don't want.  I would pay to have those stopped.''}
\item \textit{``I definitely became more concerned about how much data is taken. You don't
	realize how much of your personal data is sent to advertisers and it makes you
	more weary of downloading and using certain apps.''}
\item \textit{``I thought it was quite enlightening. I will certainly be paying more attention to what and how an app uses my data in the future.''}
\item \textit{``I definitely became more concerned about my privacy. Thank you for the wake up call.''}
\item \textit{``Good Study. Made me really think about how much of everybody's information is really out there.''}
\item \textit{``I am surprised to learn how much information could be linked to my email address.  It is like telemarketing on steroids and I would be willing to keep that info private  I think we should always have the option to keep our private info private.''}
\item \textit{``I have become a little more concerned about my privacy as some of this was new information to me. I will definitely be doing more research on this subject in the near future. Thank you for the informative study! Everything was very clear and straight forward, I appreciate the opportunity to participate.''}
%\item \textit{``I definitely learned more about how my private information is shared and will be more cautious in the future.''}
\newline
\item {\bf They are interested in using a privacy-enhancing solution:}
\item \textit{``I did not know all of that and if you developed a product I want it.''}
\item \textit{``Yes - I have been concerned, but it has been difficult to know where to start with securing my data.  I live in the US, so there is no GDPR to protect me, however I feel I can review application requests for information in a more informed manner.  I would also love to find the service you mentioned about protecting privacy of data.''}
\item \textit{``Thank you. I learned a lot from this study. I hope you are able to develop something that can help protect consumers and still allow developers to flurish.''}
\item \textit{``I would love a reliable app that limited/reduced data collection and increased privacy. Problem is that it's not possible to know which privacy apps are reliable and effective, while still allowing a service or app to be used. Even a reliable, mainstream email alternative would be good!''}

%\item {\bf Other:}
%\item \textit{``I feel that "but maybe Harmful" has broad context. to me, as someone who is concerned about my privacy, I am concerned about any data that is sent to anyone. to other's it could mean that the server-side is a bunch of hackers that are out to get all of their money. we give out our information too freely in this internet world and the majority of the people do not realize that they are doing it.''}
%\item \textit{``I feel that I pay for the phone, i pay for the service, i pay for some apps...  i don't feel that I should have to pay to keep my privacy secure.  if it is metadata and it is being used to generalize for ads or whatever, it's fine.  but if an app developer or advertiser can drill down and see my name, age, location, and income then i have a problem.''}

\end{quote}


 \begin{figure}[t!]
	\begin{center}
		%
		\subfigure{\hspace{6pt}\includegraphics[width=8.5cm]{figs/worldcloud_comments_all_workers.png}\label{fig:all_comments}}
%		\subfigure{\hspace{6pt}\includegraphics[width=7.5cm]{figs/wordcloud_master_comments.png}\label{fig:master_comments}}
		%
		\vspace{-10pt}
		\caption{Overview of main keywords extracted from 99 MTurk workers' comments} %\magenta{how many total?}}%(left) and Master user comments (right)} 
		\label{fig:comments}
		%	\vspace{-15pt}
	\end{center}   
\end{figure}






==> exposures_exposed_soups21 arxiv-2/05-conclusion.tex <==
%
\section{Conclusion \& Future Directions} \label{sec:conclusion}
%

We provided a combination of a measurement and a user study of actual PII exposed by mobile apps.  We also defined and analyzed the context (PII type, destination domain, app category/functionality, background/foreground, use of encryption vs. plain text)  where these PII exposures occur, and we distinguished between PII exposure and PII leak (which is more likely to be harmful) depending on the context. In the measurement study, we collected and analyzed a new richer dataset, which reveals  interesting PII exposures and patterns, some of which were previously unknown. Preliminary graph analysis revealed interesting patterns of apps and domains colluding to expose private information.  In the user study, we compiled the large amount of information from the measurement study into a smaller number of categories (contexts) and we asked users  to assess the privacy exposures in the actual context they appeared, w.r.t. their legitimacy and risk they pose. Most users were initially unaware of the severity and potential implications of PII exposures: they could not identify the most critical PII or context (\eg that it may be ok to share information with the application server instead of third parties, such as advertises and trackers). However, they seemed to appreciate the information they got through the study, which made them more willing to adopt privacy enhancing tools. Our analysis combines the scale and coverage of the network-based measurement study with the fine-granularity user input assessing privacy exposures in context. 

There are several directions for future work, building on the observations of this paper. First, the behavioral analysis of PII leaks at the end of Section \ref{sec:data} revealed  similarities in the way apps and destination domains extract PII from mobile devices. Those observations can be further exploited to design machine learning approaches that can detect packets with potential privacy exposures \cite{spawc_shuba, bakopoulou2019federated}, further inspect them and eventually prevent an actual leak (\eg by using real-time  tools like \anteater to block a packet or obfuscate a PII). Second, the user study showed that users are interested in and are capable of  being educated about their data, and they want to adopt better privacy practices and new tools (such as \anteater, \recon or \haystack) to enhance data transparency and privacy control. 

%We plan to make our newly developed \antShield (which was a side system contribution, but out of the main scope of this paper) and the datasets collected and analyzed in this paper available to the research community.

%%Our work in perspective.
%In this paper, we use one of the aforementioned state-of-the-art VPN-based monitoring tools, AntMonitor, to collect and analyze packet traces and the privacy exposures found therein. This approach has the advantage that it captures actual real-world privacy exposures, as opposed to e.g. potential exposures described by permissions. In addition, we compile the large volume of information from the packet traces and present it to users in a way that they can process and assess. The combination of a measurement study (volume and coverage of packet traces obtained through extensive and systematic experiments) with a user study (summarizing the information into categories, defining context, and obtaining fine-granularity feedback from users) is one of the contributions of this paper, in addition to the detailed findings of both studies as outlined in the introduction.


%Second, we developed a tool  \antShield\xspace- a system that performs, for the first time, on-device detection of \preDefLeak PII and classification of \unknownLeak PII, accurately (with higher accuracy and lower variance than state-of-the-art) and with low overhead (in real-time on the device


 %We conducted an exploratory study with real users to capture their notion of privacy awareness and to help us label different information types into legitimate and potentially harmful PII leaks. Users seem to appreciate our tutorial on mobile privacy according to their comments at the end of the study. 
%We also presented  \antShield\xspace- a system that performs, for the first time, on-device detection of \preDefLeak PII and classification of \unknownLeak PII, accurately (with higher accuracy and lower variance than state-of-the-art) and with low overhead (in real-time on the device). 
%
 %We  will make the \antShield work available to the research community, including the \antShield plugin for the \antLib on the device, the training module, and the \antShield dataset. 

% This work focused on a single device and it is the first necessary step towards enabling distributed learning of PII leakage, where multiple devices running \antShield  collaborate with each other and/or a central entity to share training data and/or classifiers. This is an important direction for future work. 
 
% We plan to conduct a second user study to collect user data from various applications is essential to train classifiers that predict PII, while providing a user friendly interface to make privacy more approachable to non tech-savvy users.
 %
 %
%If the users do not completely trust the central entity, distributed machine learning frameworks for enabling collaborative learning, while preserving user privacy, are currently an active research area.  We will consider Federated Learning  \cite{fedlearn,Bonawitz} (which enables mobile phones to collaboratively learn a shared prediction model while keeping all the training data on device, and is supported by Google); the Teacher-Student model  \cite{papernot2017semi} (ensemble-based machine learning on private datasets); and hybrid approaches such as Blender \cite{blender} (a hybrid differential privacy model where users have different privacy requirements). 





==> exposures_exposed_soups21 arxiv-2/05-related_work.tex <==
\section{Related Work} \label{sec:related}

{\bf Privacy-Preserving Tools.} There are a number of  complementary frameworks, built by different communities,  that can enhance data transparency and privacy protection on mobile devices.


{\em Permissions} are the first line of defense against unwanted access to sensitive resources. However,  they are insufficient and too coarse-grained: (i) users typically accept to install apps by default; (ii) permissions do not capture run-time behavior; (iii) they do not protect against inter-app communication and poorly documented system calls; and (iv) permissions signify {\em access} to information, which is less of a concern than {\em sharing} that information over the network.  

%Different communities have built more fine-grained tools for privacy protection, which go beyond just permissions and fit into these three broad categories.

{\em Static analysis} and application re-writing, such as \textvtt{PiOS} \cite{egele2011pios}, \textvtt{AndroidLeaks} \cite{gibler2012androidleaks}, and \cite{nanfinding2018}, suffer from the inherent imprecision of decompilation. Furthermore, static analysis does not capture representative run-time behavior and often fails to deal with native or dynamically loaded code. 

{\em Dynamic analysis} with a modified or rooted OS include \textvtt{ProtectMyPrivacy} \cite{pmp}, \taintdroid \cite{enck2014taintdroid}, and others \cite{almuhimedi2015your, phonelab, vallina2013rilanalyzer, falaki2010first, wei2012profiledroid, Wang2017}.  Such tools are powerful not suitable for mass adoption since rooting a phone or installing a custom OS is not only a daunting task for the average user, but is also strongly discouraged by wireless providers and phone manufacturers. 

{\em VPN-based network monitoring} tools use the TUN interface to capture network packets on the device and detect whenever sensitive information is sent over the networ. Over the years, their implementation has evolved from a client-server implementation \cite{meddle, recon15, antmonitor-poster-mobicom15} to a mobile-only implementation \cite{ razaghpanah2015haystack, song2015privacyguard, antmonitor-arxiv}. State-of-the-art mobile-only network monitoring tools  include \anteater \cite{antmonitor-arxiv}, \recon \cite{recon15}, \haystack \cite{razaghpanah2016haystack}, and \pguard \cite{privacyguard}) and are amenable to crowdsourcing thanks to their implementation as a mobile-only user-space app. However, to the best of our knowledge, they have been only used  so far to collect packet traces and analyze ``privacy leaks'' found therein, not for user studies. 
% In this paper, we use one of these tools, \anteater, to collect the packets used in our measurement study, but we also use these data to design a user study.


%Static analysis and application re-writing \cite{nanfinding2018, gibler2012androidleaks, egele2011pios, Wang2017}, (ii) dynamic analysis with a modified or rooted OS \cite{enck2014taintdroid, phonelab, vallina2013rilanalyzer, falaki2010first, wei2012profiledroid, Wang2017}, and (iii) VPN-based network monitoring \cite{meddle, antmonitor-poster-mobicom15, razaghpanah2015haystack, song2015privacyguard, recon15, antmonitor-arxiv, antshield-arxiv}. Tools that fall into the first category, such as \textvtt{PiOS} \cite{egele2011pios}, \textvtt{AndroidLeaks} \cite{gibler2012androidleaks}, and \cite{nanfinding2018}, suffer from the inherent imprecision of decompilation. Furthermore, static analysis does not capture representative run-time behavior, and often fails to deal with native or dynamically loaded code. Tools of the second category include \textvtt{ProtectMyPrivacy} \cite{pmp}, \taintdroid \cite{enck2014taintdroid}, and \cite{almuhimedi2015your}. Such tools are not suitable for mass adoption since rooting a phone or installing a custom OS is not only a daunting task for the average user, but is also strongly discouraged by wireless providers and phone manufacturers. Tools of the third category (\anteater \cite{antmonitor-arxiv}, \recon \cite{recon15}, \haystack \cite{razaghpanah2016haystack}, and \pguard \cite{privacyguard}) are user-friendly as they come in a form of a user-space app that detects whenever sensitive information is sent over the network. However, these most-promising tools have largely remained unstudied.



{\bf Privacy ``Leak'' Datasets.} The aforementioned tools have been used before to collect datasets containing privacy ``leaks'' (see Footnote 1 for terminology) from mobile devices. Most closely related to this paper, the VPN-based monitoring tools only used so far to collect packet traces and analyze ``privacy leaks'' found therein, not for user studies.  \recon \cite{recon15} collected packet traces to train machine learning classifiers for predicting PII exposures. Razaghpanah et al. \cite{vallina2018tracking} collected cases of PII exposures from thousands of users using the \haystack app and used that data to find new advertising and tracking services. Finally, the longitudinal study of PII exposures in \cite{Ren2018} demonstrates how privacy evolves across different app versions in Android. %In particular, they used automated  interacting with 500 apps to generate the data when testing different versions of the same apps. %and they check the validility of their data by comparing real user interaction available through Lumen.


{\bf User Studies.} 
Several experimental studies have analyzed mobile app behavior and several users studies have analyzed user interactions and mobile usage (\eg Mehrotra et al.  \cite{Mehrotra2017}, Tian et al. \cite{Tian2013}, \textvtt{EarlyBird} \cite{Wang2015} and Xu et al. \cite{Xu:2011:IDU:2068816.2068847}). Most closely related to this paper, are user studies that focus specifically on privacy.  
%\blue{The work in \cite{Li:2017:PET:3139486.3130941} proposes a tool for accessing personal data as a stream based on functional programming. They analyze 100 popular apps from Google Play and study which of them do not need full access to the raw data but they require permissions in order to access them. They support different granularity levels depending on the app. The type of information they consider are: Location, Microphone, Contacts, Messages, Files, etc. They do not focus on the PII types we do.}

Permissions and how users interact with them have been extensively studied in \cite{Ismail2017, Jorgensen2015, wang2015investigating, almuhimedi2015your, Lin2012, Liu2016}. Almuhimedi et al. \cite{almuhimedi2015your} studied how sending users privacy nudges affected their permission settings. Wang et al. \cite{wang2015investigating} studied user decisions when presented with permission settings that are separated between apps and ad libraries. More recently, Ismail et al. \cite{Ismail2017} showed that it is possible to maintain app usability even when disallowing certain permissions. Chitkara et al. proposed a retrofitted Android system, \textvtt{ProtectMyPrivacy} \cite{pmp}, that allows users to make fewer privacy decisions by setting permissions based on third-party libraries instead of applications. 

Taking a different approach,  \textvtt{PrivacyStreams} \cite{Li:2017:PET:3139486.3130941} proposes and evaluates (with a user study) a tool for developers to write code in a more privacy-preserving way. In the web ecosystem, the work in \cite{Rao2016} studies online privacy in websites to identify mismatched user expectations and the factors that impact these mismatches. The work by Kleek et al. \cite{van2017better} is closest to our work in that they use information captured from network monitoring to see if it influences users' decisions to install apps. Unlike their work, however, we are interested in learning what users would do if given more fine-grained control over their data. 

{\bf Our work in perspective.} In this paper, we use one of the aforementioned state-of-the-art VPN-based monitoring tools, \anteater \cite{antmonitor-page, antmonitor-arxiv}, to collect and analyze packet traces and the privacy exposures found therein. This approach has the advantage that it captures actual real-world privacy exposures, as opposed to \eg potential exposures described by permissions. In addition, we compile the large volume of information from the packet traces and present it to users in a way that they can process and assess. The combination of a measurement study (volume and coverage of packet traces obtained through extensive and systematic experiments) with a user study (summarizing the information into  categories, defining context, and obtaining fine-granularity feedback from users) is one of the contributions of this paper, in addition to the detailed findings of both studies as outlined in the introduction.


%In our work, we attempt to remedy this by capturing how different users react to each PII type being sent to various destinations (advertisers and/or app developers) by apps from various categories, based on real cases from a dataset that we collected. 

% NOTE: this paragraph is summarized above
%\magenta{[Why was this paragraph commented out?]}Various works used crowdsourcing to study users' behavior regarding mobile apps and privacy. A related work is proposed in \cite{Lin2012}, where the authors measured users' perceptions of what actions are legitimate and how threatened they feel by certain apps' actions. The goal of this work is to introduce a new model for privacy called ``privacy as expectations''. This new model generates a new interface that includes a summary of how other users feel for the resources required by an app before downloading this particular app. That way, a user can either agree to download an app or change their mind by reading what other users think. Although this work is similar to our user study, they used permissions and a limited number of sensitive resources (unique device ID, contact list, network location, GPS location) and we used an extensive list of 16 unique PII types in this work. A more recent work proposed by \cite{Jorgensen2015} captures via crowdsourcing the risks of installing an app. In particular, they assigned card sorting tasks to experts and novices that includes categorizing  permissions in four dimensions: (i) personal information privacy, (ii) monetary risk, (iii) device availability/stability and (iv) data integrity for the card sorting task. Another similar work is proposed by \cite{Ismail2017}, where the authors study mobile apps permissions settings via crowdsourcing. They examine how the usability of certains apps is affected by disabling certain permissions that are required for their functionality. Furthermore, the work in \cite{Rao2016} studies online privacy in websites to identify mismatched user expectations and the factors that impact these mismatches. Their goal is to generate a simplified version of privacy notices for websites to faciliate the undestanding of privacy risks online.

% Overall, our goal is to educate these users about mobile privacy, capture their concerns about various types of sensitive information leaked and hopefully increase their awaness to adapt their behavior as users. 




\begin{comment}
Different communities are working on improving data transparency and exposing or preventing potential privacy leaks. {\em Permissions} are useful but not sufficient: . Using a {\em custom OS}  or a rooted phone one can get access to fine-grained information on the device, including network traffic.  \textvtt{Phonelab} \cite{phonelab} and others \cite{vallina2013rilanalyzer, wei2012profiledroid} use packet capturing APIs such as \textvtt{tcpdump} or \textvtt{iptables-log}. These are powerful  but  inherently limited to small scale-deployment as the overwhelming majority of  users do not have rooted phones,  and wireless providers and phone manufacturers strongly discourage rooting. The same limitation applies to approaches that use a custom OS to dynamically intercept leaks (\eg\xspace \textvtt{\taintdroid} \cite{enck2014taintdroid}) or permission requests to certain resources (\eg\xspace \textvtt{\appfence} \cite{hornyack2011thesedroids}).
%


Within the network measurements community, a number of prior works \cite{meddle, recon15, antmonitor-arxiv, antmonitor-poster-mobicom15, razaghpanah2016haystack}  %
have looked for personal information  leaks in network traffic. %
This includes monitoring in the middle of the network (as in \meddle  \cite{meddle} and \recon \cite{recon15})  or on the device  itself (as in  \anteater (\cite{antmonitor-arxiv, antmonitor-poster-mobicom15}) and \textvtt{Lumen} (a.k.a. \haystack) \cite{razaghpanah2016haystack}).  \anteater and  \textvtt{Lumen} detect leaks on the device, but require a blacklist of strings (potential PII leaks) known a priori to search for; therefore, they are unable to detect leakage of information that changes dynamically or is not part of the list. 

To remedy this limitation, \recon recently applied machine learning techniques  to predict whether or not a given packet contains PII  \cite{recon15}. They broke packets into words based on delimiters (\eg `?', `=', `:') and then used these words as features in classification. Various methods were used to ensure that the PII themselves and strings that occur too often or too infrequently are not part of the feature list, see \cite{recon15} for details.
To decide whether or not a packet contains PII (a binary classification problem), \recon used the Java Weka library's \cite{hall2009weka} C4.5 Decision Tree (DT), and then heuristics for extracting the type of leak. To improve classification accuracy \recon built specialized classifiers for each destination domain that received enough data to train such a classifier. For the rest of the domains, a {\em general} classifier was built. For the heuristic step, \recon maintained a list of probabilities that a particular key-word corresponds to a PII value. For each PII type, the probability was calculated by taking the number of times the key was present in a packet with the given PII, and dividing it by the number of times the key appeared in all packets. During PII extraction, \recon looked for keys with probability higher than an empirically computed threshold. Their code and dataset are available at \cite{recondata}.
%

\recon is the closest to our work, thus we use it as our baseline for comparison throughout the paper.  The  key difference lies in the centralized vs distributed approach. \recon collected its datasets in the middle of the network, trained and applied the classifiers in a centralized way. \antShield operates on the device, which poses unique system challenges and learning opportunities, and paves the way for truly distributed learning of privacy leakage.
\end{comment}




%\magenta{[Check user studies by Narseo longitutal NDSS, and check last Ubicomp and PETS for user studies]}

%In \cite{Xu2011}, the authors study app usage in the U.S. based on anonymized HTTP signatures. 





==> exposures_exposed_soups21 arxiv-2/acknowledgements.tex <==
\section{Acknowledgments}\label{sec:acknowledgements}

%This work has been partially funded by NSF Awards 1649372 and 1526736. E. Bakopoulou has been partially supported by H. Samueli, Networked Systems, and Broadcom Foundation Fellowships. A. Shuba has been supported by ...
We would like to thank Milad Asgari Mehrabadi for providing figures 2 and 3 for this paper.

This work has been supported by NSF Awards 1649372, 1815666, 1900654 and by a UCI Proof-of-Concept Award in 2017. E. Bakopoulou has also been supported by the Broadcom Foundation and Henry Samueli fellowships. A. Shuba  has also been supported by an ARCS Fellowship.
